The Single-Phase ProtoDUNE Technical Design Report

ProtoDUNE-SP is the single-phase DUNE Far Detector prototype that is under construction and will be operated at the CERN Neutrino Platform (NP) starting in 2018. ProtoDUNE-SP, a crucial part of the DUNE effort towards the construction of the first DUNE 10-kt fiducial mass far detector module (17 kt total LAr mass), is a significant experiment in its own right. With a total liquid argon (LAr) mass of 0.77 kt, it represents the largest monolithic single-phase LArTPC detector to be built to date. It's technical design is given in this report.

==> authors.tex <==
% The author list in authblk format
% This file was generated on Jan. 26, 2016, 5 p.m. 
% The collaboration listed is as it was on the date: 2016-01-26.
% Retrieved from: dune.bnl.gov/people/members/export/?filename=author-payload-authblk.tex&amp;date=now
% This file was generatd, do not edit this file!
% Contact Maury Goodman for any changes.






\author[102]{B.~Abi}
\author[43]{R.~Acciarri}
\author[9]{M.~A.~Acero}
\author[43]{M.~Adamowski}
\author[143]{C.~Adams}
\author[43]{P.~Adamson}
\author[134]{Z.~Ahmad}
\author[43]{C.~H.~Albright}
\author[120]{T.~Alion}
\author[130]{E.~Amador}
\author[7]{J.~Anderson}
\author[43]{K.~Anderson}
\author[77]{C.~Andreopoulos}
\author[43]{M.~P.~Andrews}
\author[43]{R.~A.~Andrews}
\author[62]{I.~Anghel}
\author[99]{J.~d.~Anjos}
\author[136]{A.~Ankowski}
\author[73]{M.~Antonello}
\author[31]{A.~Aranda~Fernandez}
\author[12]{A.~Ariga}
\author[12]{T.~Ariga}
\author[76]{D.~Aristizabal}
\author[87]{E.~Arrieta-Diaz}
\author[130]{J.~Asaadi}
\author[103]{D.~Asner}
\author[5]{M.~S.~Athar}
\author[12]{M.~Auger}
\author[29]{A.~Aurisano}
\author[69]{V.~Aushev}
\author[63]{D.~Autiero}
\author[130]{M.~Avila}
\author[102]{F.~Azfar}
\author[138]{J.~J.~Back}
\author[122]{X.~Bai}
\author[106]{B.~Baibussinov}
\author[127]{M.~Baird}
\author[141]{A.~B.~Balantekin}
\author[43]{B.~Baller}
\author[41]{P.~Ballett}
\author[52]{B.~Bambah}
\author[107]{M.~Bansal}
\author[107]{S.~Bansal}
\author[138]{G.~J.~Barker}
\author[102]{G.~Barr}
\author[109]{N.~Barros}
\author[16]{B.~Bartosz}
\author[79]{L.~Bartoszek}
\author[101]{A.~Bashyal}
\author[102]{M.~Bass}
\author[132]{F.~Bay}
\author[100]{J.~F.~Beacom}
\author[107]{B.~R.~Behera}
\author[110]{G.~Bellettini}
\author[26]{V.~Bellini}
\author[16]{O.~Beltramello}
\author[16]{N.~Benekos}
\author[108]{P.~A.~Benetti}
\author[114]{A.~Bercellie}
\author[43]{E.~Berman}
\author[20]{H.~Berns}
\author[43]{R.~Bernstein}
\author[16]{S.~Bertolucci}
\author[49]{B.~Bhandari}
\author[107]{V.~Bhatnagar}
\author[60]{B.~Bhuyan}
\author[90]{J.~Bian}
\author[43]{K.~Biery}
\author[14]{M.~Bishai}
\author[127]{T.~Blackburn}
\author[74]{A.~Blake}
\author[13]{F.~d.~M.~Blaszczyk}
\author[83]{E.~Blaufuss}
\author[124]{B.~Bleakley}
\author[28]{E.~Blucher}
\author[43]{V.~Bocean}
\author[108]{F.~Boffelli}
\author[79]{J.~Boissevain}
\author[117]{S.~Bolognesi}
\author[66]{T.~Bolton}
\author[89]{M.~Bonesini}
\author[33]{T.~Boone}
\author[118]{C.~Booth}
\author[53]{S.~Bordoni}
\author[69]{M.~Borysova}
\author[53]{B.~Bourguille}
\author[138]{S.~B.~Boyd}
\author[74]{D.~Brailsford}
\author[130]{A.~Brandt}
\author[16]{J.~Bremer}
\author[43]{S.~Brice}
\author[87]{C.~Bromberg}
\author[34]{G.~Brooijmans}
\author[130]{G.~Brown}
\author[43]{G.~Brunetti}
\author[43]{X.~Bu}
\author[33]{N.~Buchanan}
\author[114]{H.~Budd}
\author[129]{B.~Bugg}
\author[75]{P.~Calafiura}
\author[108]{E.~Calligarich}
\author[17]{E.~Calvo}
\author[34]{L.~Camilleri}
\author[78]{M.~Campanelli}
\author[146]{C.~Cantini}
\author[43]{B.~Carls}
\author[78]{M.~Cascella}
\author[44]{C.~Castromonte}
\author[62]{E.~Catano~Mur}
\author[43]{F.~Cavanna}
\author[106]{S.~Centro}
\author[135]{A.~Cervera~Villanueva}
\author[16]{M.~Chalifour}
\author[126]{M.~Chamizo~Llatas}
\author[11]{V.~B.~Chandratre}
\author[130]{A.~Chatterjee}
\author[43]{S.~Chattopadhyay}
\author[134]{S.~Chattopadhyay}
\author[63]{L.~Chaussard}
\author[52]{S.~Chembra}
\author[14]{H.~Chen}
\author[14]{K.~Chen}
\author[21]{M.~Chen}
\author[33]{D.~Cherdack}
\author[34]{C.~Chi}
\author[43]{S.~Childress}
\author[47]{S.~Choubey}
\author[38]{B.~C.~Choudhary}
\author[77]{G.~Christodoulou}
\author[122]{C.~Christofferson}
\author[103]{E.~Church}
\author[82]{D.~Cianci}
\author[125]{T.~Coan}
\author[93]{A.~Cocco}
\author[58]{P.~Cole}
\author[84]{G.~Collin}
\author[84]{J.~M.~Conrad}
\author[115]{M.~Convery}
\author[122]{R.~Corey}
\author[122]{L.~Corwin}
\author[7]{J.~Cranshaw}
\author[34]{J.~I.~Crespo-Anad\'on}
\author[146]{P.~Crivelli}
\author[90]{D.~Cronin-Hennessy}
\author[89]{A.~Curioni}
\author[28]{J.~Cushing}
\author[14]{D.~L.~Adams}
\author[58]{D.~Dale}
\author[60]{S.~R.~Das}
\author[116]{T.~Davenne}
\author[61]{G.~S.~Davies}
\author[127]{J.~Davies}
\author[2]{J.~Dawson}
\author[130]{K.~De}
\author[97]{A.~de~Gouvea}
\author[102]{J.~K.~de~Jong}
\author[92]{P.~de~Jong}
\author[7]{P.~De~Lurgio}
\author[92]{M.~Decowski}
\author[117]{A.~Delbart}
\author[116]{C.~Densham}
\author[7]{R.~Dharmapalan}
\author[107]{N.~Dhingra}
\author[146]{S.~Di~Luise}
\author[8]{M.~Diamantopoulou}
\author[61]{J.~S.~Diaz}
\author[114]{G.~Diaz~Bautista}
\author[14]{M.~Diwan}
\author[7]{Z.~Djurcic}
\author[14]{J.~Dolph}
\author[7]{G.~Drake}
\author[72]{D.~Duchesneau}
\author[141]{M.~Duvernois}
\author[120]{H.~Duyang}
\author[75]{D.~A.~Dwyer}
\author[48]{S.~Dye}
\author[111]{S.~Dytman}
\author[115]{B.~Eberly}
\author[50]{R.~Edgecock}
\author[87]{D.~Edmunds}
\author[79]{S.~Elliott}
\author[21]{M.~Elnimr}
\author[117]{S.~Emery}
\author[105]{E.~Endress}
\author[83]{S.~Eno}
\author[12]{A.~Ereditato}
\author[43]{C.~O.~Escobar}
\author[82]{J.~Evans}
\author[108]{A.~Falcone}
\author[127]{L.~Falk}
\author[130]{A.~Farbin}
\author[106]{C.~Farnese}
\author[57]{Y.~Farzan}
\author[106]{A.~Fava}
\author[18]{L.~Favilli}
\author[83]{J.~Felde}
\author[46]{J.~Felix}
\author[3]{S.~Fernandes}
\author[43]{L.~Fields}
\author[74]{A.~Finch}
\author[116]{M.~Fitton}
\author[143]{B.~Fleming}
\author[58]{T.~Forest}
\author[40]{J.~Fowler}
\author[61]{W.~Fox}
\author[14]{J.~Fried}
\author[115]{A.~Friedland}
\author[43]{S.~Fuess}
\author[75]{B.~Fujikawa}
\author[105]{A.~Gago}
\author[133]{H.~Gallagher}
\author[63]{S.~Galymov}
\author[118]{T.~Gamble}
\author[47]{R.~Gandhi}
\author[82]{D.~Garcia-Gamez}
\author[20]{S.~Gardiner}
\author[79]{G.~Garvey}
\author[75]{V.~M.~Gehman}
\author[146]{A.~Gendotti}
\author[14]{G.~d.~Geronimo}
\author[78]{C.~Ghag}
\author[47]{P.~Ghoshal}
\author[106]{D.~Gibin}
\author[17]{I.~Gil-Botella}
\author[14]{R.~Gill}
\author[25]{D.~Girardelli}
\author[55]{A.~Giri}
\author[109]{S.~Glavin}
\author[12]{D.~Goeldi}
\author[66]{S.~Golapinni}
\author[96]{M.~Gold}
\author[44]{R.~A.~Gomes}
\author[135]{J.~J.~Gomez~Cadenas}
\author[7]{M.~C.~Goodman}
\author[56]{D.~Gorbunov}
\author[47]{S.~Goswami}
\author[111]{N.~Graf}
\author[115]{N.~Graf}
\author[115]{M.~Graham}
\author[143]{E.~Gramelini}
\author[91]{R.~Gran}
\author[20]{C.~Grant}
\author[138]{N.~Grant}
\author[26]{V.~Greco}
\author[43]{H.~Greenlee}
\author[141]{L.~Greenler}
\author[29]{M.~Groh}
\author[109]{S.~Grullon}
\author[74]{T.~Grundy}
\author[137]{K.~Grzelak}
\author[79]{E.~Guardincerri}
\author[136]{E.~Guarnaccia}
\author[42]{G.~P.~Guedes}
\author[102]{R.~Guenette}
\author[106]{A.~Guglielmi}
\author[91]{A.~T.~Habig}
\author[14]{R.~W.~Hackenburg}
\author[143]{A.~Hackenburg}
\author[130]{H.~Hadavand}
\author[12]{R.~Haenni}
\author[43]{A.~Hahn}
\author[138]{M.~D.~Haigh}
\author[79]{T.~Haines}
\author[43]{T.~Hamernik}
\author[129]{T.~Handler}
\author[14]{S.~Hans}
\author[43]{D.~Harris}
\author[127]{J.~Hartnell}
\author[68]{T.~Hasegawa}
\author[43]{R.~Hatcher}
\author[129]{A.~Hatzikoutelis}
\author[43]{S.~Hays}
\author[13]{E.~Hazen}
\author[123]{M.~Headley}
\author[43]{A.~Heavey}
\author[143]{K.~Heeger}
\author[123]{J.~Heise}
\author[77]{K.~Hennessy}
\author[82]{J.~Hewes}
\author[49]{A.~Higuera}
\author[58]{T.~Hill}
\author[43]{A.~Himmel}
\author[33]{M.~Hogan}
\author[25]{P.~Holanda}
\author[78]{A.~Holin}
\author[74]{W.~Honey}
\author[146]{S.~Horikawa}
\author[66]{G.~Horton-Smith}
\author[61]{B.~Howard}
\author[43]{J.~Howell}
\author[43]{P.~Hurh}
\author[87]{J.~Huston}
\author[43]{J.~Hylen}
\author[80]{R.~Imlay}
\author[80]{J.~Insler}
\author[108]{G.~Introzzi}
\author[144]{D.~Ioanisyan}
\author[144]{A.~Ioannisian}
\author[114]{K.~Iwamoto}
\author[135]{A.~Izmaylov}
\author[130]{C.~Jackson}
\author[14]{D.~E.~Jaffe}
\author[43]{C.~James}
\author[43]{E.~James}
\author[36]{F.~Jediny}
\author[136]{C.~Jen}
\author[107]{A.~Jhingan}
\author[17]{S.~Jim\'enez}
\author[126]{J.~H.~Jo}
\author[43]{M.~Johnson}
\author[29]{R.~Johnson}
\author[43]{J.~Johnstone}
\author[84]{B.~J.~Jones}
\author[14]{J.~Joshi}
\author[43]{H.~Jostlein}
\author[126]{C.~K.~Jung}
\author[43]{T.~Junk}
\author[59]{A.~Kaboth}
\author[133]{T.~Kafka}
\author[136]{L.~Kalousis}
\author[129]{Y.~Kamyshkov}
\author[82]{G.~Karagiorgi}
\author[8]{D.~Karasavvas}
\author[72]{Y.~Karyotakis}
\author[107]{A.~Kaur}
\author[107]{P.~Kaur}
\author[43]{B.~Kayser}
\author[144]{N.~Kazaryan}
\author[13]{E.~Kearns}
\author[109]{P.~Keener}
\author[130]{S.~Kemboi}
\author[25]{E.~Kemp}
\author[14]{S.~H.~Kettell}
\author[56]{M.~Khabibullin}
\author[58]{M.~Khandaker}
\author[56]{A.~Khotjantsev}
\author[14]{B.~Kirby}
\author[43]{M.~Kirby}
\author[109]{J.~Klein}
\author[43]{T.~Kobilarcik}
\author[132]{B.~Kocaman}
\author[19]{S.~Kohn}
\author[43]{G.~Koizumi}
\author[56]{A.~Kopylov}
\author[140]{M.~Kordosky}
\author[74]{L.~Kormos}
\author[16]{U.~Kose}
\author[61]{V.~A.~Kosteleck\'y}
\author[19]{M.~Kramer}
\author[12]{I.~Kreslo}
\author[21]{W.~Kropp}
\author[56]{Y.~Kudenko}
\author[118]{V.~A.~Kudryavtsev}
\author[56]{S.~Kulagin}
\author[107]{A.~Kumar}
\author[70]{G.~K.~Kumar}
\author[48]{J.~Kumar}
\author[107]{L.~Kumar}
\author[80]{T.~Kutter}
\author[132]{M.~K\"OPR\"U}
\author[130]{B.~T.~Lam}
\author[3]{A.~Laminack}
\author[109]{K.~Lande}
\author[39]{C.~Lane}
\author[131]{K.~Lang}
\author[14]{F.~Lanni}
\author[48]{J.~Learned}
\author[43]{P.~Lebrun}
\author[79]{D.~Lee}
\author[114]{H.~Lee}
\author[43]{W.~M.~Lee}
\author[1]{M.~A.~Leigui~de~Oliveira}
\author[43]{Q.~Li}
\author[14]{S.~Li}
\author[100]{S.~W.~Li}
\author[126]{X.~Li}
\author[14]{Y.~Li}
\author[40]{Z.~Li}
\author[75]{C.~S.~Lin}
\author[33]{S.~Lin}
\author[14]{J.~Ling}
\author[136]{J.~Link}
\author[32]{Z.~Liptak}
\author[14]{D.~Lissauer}
\author[14]{L.~Littenberg}
\author[54]{B.~Littlejohn}
\author[79]{Q.~Liu}
\author[125]{T.~Liu}
\author[43]{S.~Lockwitz}
\author[43]{N.~Lockyer}
\author[75]{T.~Loew}
\author[15]{M.~Lokajicek}
\author[59]{K.~Long}
\author[65]{K.~Loo}
\author[43]{M.~D.~L.~Lopes}
\author[32]{J.~P.~Lopez}
\author[12]{D.~Lorca}
\author[98]{J.~Losecco}
\author[79]{W.~Louis}
\author[61]{J.~Lowery}
\author[12]{M.~Luethi}
\author[19]{K.~Luk}
\author[43]{B.~Lundberg}
\author[43]{T.~Lundin}
\author[143]{X.~Luo}
\author[53]{T.~Lux}
\author[43]{J.~Lykken}
\author[65]{J.~Maalampi}
\author[73]{A.~A.~Machado}
\author[43]{J.~R.~Macier}
\author[7]{S.~Magill}
\author[14]{G.~Mahler}
\author[87]{K.~Mahn}
\author[59]{M.~Malek}
\author[11]{S.~Malhotra}
\author[7]{D.~Malon}
\author[26]{F.~Mammoliti}
\author[38]{S.~K.~Mandal}
\author[52]{S.~Mandodi}
\author[114]{S.~L.~Manly}
\author[133]{A.~Mann}
\author[43]{A.~Marchionni}
\author[14]{W.~Marciano}
\author[136]{C.~Mariani}
\author[48]{J.~Maricic}
\author[32]{A.~D.~Marino}
\author[90]{M.~Marshak}
\author[114]{C.~Marshall}
\author[24]{J.~Marshall}
\author[63]{J.~Marteau}
\author[102]{J.~Martin-Albo}
\author[54]{D.~Martinez}
\author[48]{S.~Matsuno}
\author[80]{J.~Matthews}
\author[77]{K.~Mavrokoridis}
\author[144]{D.~Mayilyan}
\author[89]{R.~Mazza}
\author[117]{E.~Mazzucato}
\author[77]{N.~McCauley}
\author[43]{E.~McCluskey}
\author[118]{N.~McConkey}
\author[112]{K.~McDonald}
\author[114]{K.~S.~McFarland}
\author[114]{A.~M.~McGowan}
\author[126]{C.~McGrew}
\author[98]{S.~R.~McGuinness}
\author[140]{R.~McKeown}
\author[58]{D.~McNulty}
\author[124]{R.~McTaggart}
\author[56]{A.~Mefodiev}
\author[33]{M.~Mehrian}
\author[95]{P.~Mehta}
\author[121]{D.~Mei}
\author[135]{O.~Mena}
\author[145]{S.~Menary}
\author[85]{H.~Mendez}
\author[108]{A.~Menegolli}
\author[106]{G.~Meng}
\author[3]{D.~Mertins}
\author[61]{M.~Messier}
\author[80]{W.~Metcalf}
\author[61]{M.~Mewes}
\author[139]{H.~Meyer}
\author[43]{T.~Miao}
\author[48]{R.~Milincic}
\author[90]{W.~Miller}
\author[79]{G.~Mills}
\author[56]{O.~Mineev}
\author[30]{O.~Miranda}
\author[43]{C.~S.~Mishra}
\author[120]{S.~R.~Mishra}
\author[51]{B.~Mitrica}
\author[16]{D.~Mladenov}
\author[104]{I.~Mocioiu}
\author[52]{R.~Mohanta}
\author[43]{N.~Mokhov}
\author[16]{C.~Montanari}
\author[43]{D.~Montanari}
\author[84]{J.~Moon}
\author[14]{M.~Mooney}
\author[43]{C.~Moore}
\author[43]{J.~Morfin}
\author[138]{B.~Morgan}
\author[49]{C.~Morris}
\author[14]{W.~Morse}
\author[84]{Z.~Moss}
\author[43]{C.~Mossey}
\author[1]{C.~A.~Moura}
\author[86]{J.~Mousseau}
\author[23]{L.~Mualem}
\author[139]{M.~Muether}
\author[61]{S.~Mufson}
\author[146]{S.~Murphy}
\author[61]{J.~Musser}
\author[130]{R.~Musser}
\author[127]{D.~P.~M\'endez}
\author[75]{Y.~Nakajima}
\author[111]{D.~Naples}
\author[9]{J.~Navarro}
\author[17]{D.~Navas}
\author[140]{J.~Nelson}
\author[16]{M.~Nessi}
\author[109]{M.~Newcomer}
\author[130]{K.~T.~T.~Nguyen}
\author[78]{R.~Nichol}
\author[116]{T.~C.~Nicholls}
\author[146]{K.~Nikolics}
\author[61]{E.~Niner}
\author[43]{B.~Norris}
\author[16]{F.~Noto}
\author[14]{P.~Novakova}
\author[135]{P.~Novella}
\author[74]{J.~Nowak}
\author[25]{M.~S.~Nunes}
\author[74]{H.~O'Keeffe}
\author[24]{R.~Oldeman}
\author[25]{R.~Oliveira}
\author[133]{T.~Olson}
\author[69]{Y.~Onishchuk}
\author[43]{J.~Osta}
\author[56]{T.~Ovsjannikova}
\author[87]{B.~Page}
\author[48]{S.~Pakvasa}
\author[118]{S.~Pal}
\author[43]{O.~Palamara}
\author[43]{J.~Paley}
\author[17]{C.~Palomares}
\author[20]{E.~Pantic}
\author[111]{V.~Paolone}
\author[43]{V.~Papadimitriou}
\author[136]{J.~Park}
\author[43]{S.~Parke}
\author[14]{Z.~Parsa}
\author[41]{S.~Pascoli}
\author[23]{R.~Patterson}
\author[75]{S.~J.~Patton}
\author[2]{T.~Patzak}
\author[141]{B.~Paulos}
\author[1]{L.~Paulucci}
\author[43]{Z.~Pavlovic}
\author[90]{G.~Pawloski}
\author[127]{S.~Peeters}
\author[63]{E.~Pennacchio}
\author[78]{A.~Perch}
\author[43]{G.~N.~Perdue}
\author[146]{L.~Periale}
\author[118]{J.~D.~Perkin}
\author[72]{H.~Pessard}
\author[43]{G.~Petrillo}
\author[120]{R.~Petti}
\author[122]{A.~Petukhov}
\author[106]{F.~Pietropaolo}
\author[43]{R.~Plunkett}
\author[90]{R.~Poling}
\author[43]{M.~Popovic}
\author[43]{S.~Pordes}
\author[14]{M.~Potekhin}
\author[26]{R.~Potenza}
\author[64]{B.~Potukuchi}
\author[121]{N.~Poudyal}
\author[43]{O.~Prokofiev}
\author[107]{N.~Pruthi}
\author[94]{P.~Przewlocki}
\author[43]{D.~Pushka}
\author[14]{X.~Qian}
\author[43]{J.~L.~Raaf}
\author[6]{R.~Raboanary}
\author[14]{V.~Radeka}
\author[140]{A.~Radovic}
\author[43]{I.~Rakhno}
\author[6]{H.~T.~Rakotondramanana}
\author[6]{L.~Rakotondravohitra}
\author[138]{Y.~A.~Ramachers}
\author[43]{R.~Rameika}
\author[79]{J.~Ramsey}
\author[108]{A.~Rappoldi}
\author[108]{G.~Raselli}
\author[74]{P.~Ratoff}
\author[43]{B.~Rebel}
\author[146]{C.~Regenfus}
\author[122]{J.~Reichenbacher}
\author[43]{D.~Reitzner}
\author[72]{A.~Remoto}
\author[49]{A.~Renshaw}
\author[14]{S.~Rescia}
\author[118]{M.~Richardson}
\author[79]{K.~Rielage}
\author[43]{K.~Riesselmann}
\author[118]{M.~Robinson}
\author[115]{L.~Rochester}
\author[25]{O.~B.~Rodrigues}
\author[114]{P.~Rodrigues}
\author[86]{B.~Roe}
\author[48]{M.~Rosen}
\author[43]{R.~M.~Roser}
\author[41]{M.~Ross-Lonergan}
\author[108]{M.~Rossella}
\author[146]{A.~Rubbia}
\author[45]{C.~Rubbia}
\author[43]{R.~Rucinski}
\author[12]{C.~Rudolph~von~Rohr}
\author[143]{B.~Russell}
\author[114]{D.~Ruterbories}
\author[78]{R.~Saakyan}
\author[55]{N.~Sahu}
\author[88]{P.~Sala}
\author[14]{N.~Samios}
\author[53]{F.~Sanchez}
\author[62]{M.~Sanchez}
\author[112]{B.~Sands}
\author[85]{S.~Santana}
\author[17]{R.~Santorelli}
\author[126]{G.~Santucci}
\author[8]{N.~Saoulidou}
\author[88]{A.~Scaramelli}
\author[101]{H.~Schellman}
\author[43]{P.~Schlabach}
\author[43]{R.~Schmitt}
\author[28]{D.~Schmitz}
\author[133]{J.~Schneps}
\author[40]{K.~Scholberg}
\author[43]{A.~Schukraft}
\author[33]{J.~Schwehr}
\author[73]{E.~Segreto}
\author[109]{S.~Seibert}
\author[62]{J.~A.~Sepulveda-Quiroz}
\author[146]{F.~Sergiampietri}
\author[43]{L.~Sexton-Kennedy}
\author[146]{D.~Sgalaberna}
\author[34]{M.~H.~Shaevitz}
\author[107]{J.~Shahi}
\author[130]{S.~Shahsavarani}
\author[43]{P.~Shanahan}
\author[47]{S.~U.~Shankar}
\author[14]{R.~Sharma}
\author[113]{R.~K.~Sharma}
\author[43]{T.~Shaw}
\author[126]{R.~Shrock}
\author[69]{I.~Shyrma}
\author[14]{N.~Simos}
\author[12]{J.~Sinclair}
\author[40]{G.~Sinev}
\author[107]{I.~Singh}
\author[107]{J.~Singh}
\author[81]{J.~Singh}
\author[10]{V.~Singh}
\author[79]{G.~Sinnis}
\author[34]{F.~W.~Sippach}
\author[16]{D.~Smargianaki}
\author[21]{M.~Smy}
\author[43]{E.~Snider}
\author[54]{P.~Snopok}
\author[142]{J.~Sobczyk}
\author[21]{H.~Sobel}
\author[128]{M.~Soderberg}
\author[139]{N.~Solomey}
\author[79]{W.~Sondheim}
\author[135]{M.~Sorel}
\author[29]{A.~Sousa}
\author[27]{K.~Soustruznik}
\author[86]{J.~Spitz}
\author[118]{N.~J.~Spooner}
\author[43]{M.~Stancari}
\author[3]{I.~Stancu}
\author[16]{D.~Stefan}
\author[75]{H.~M.~Steiner}
\author[14]{J.~Stewart}
\author[122]{J.~Stock}
\author[51]{S.~Stoica}
\author[13]{J.~Stone}
\author[43]{J.~Strait}
\author[28]{M.~Strait}
\author[43]{T.~Strauss}
\author[43]{S.~Striganov}
\author[94]{R.~Sulej}
\author[83]{G.~Sullivan}
\author[48]{Y.~Sun}
\author[7]{L.~Suter}
\author[26]{C.~M.~Sutera}
\author[20]{R.~Svoboda}
\author[37]{B.~Szczerbinska}
\author[82]{A.~Szelc}
\author[82]{S.~S\"oldner-Rembold}
\author[127]{M.~Tamsett}
\author[43]{S.~Tariq}
\author[58]{E.~Tatar}
\author[61]{R.~Tayloe}
\author[79]{C.~Taylor}
\author[34]{K.~Terao}
\author[118]{M.~Thiesse}
\author[78]{J.~Thomas}
\author[118]{L.~F.~Thompson}
\author[24]{M.~Thomson}
\author[14]{C.~Thorn}
\author[116]{M.~Thorpe}
\author[120]{X.~Tian}
\author[122]{D.~Tiedt}
\author[43]{S.~C.~Timm}
\author[2]{A.~Tonazzo}
\author[43]{T.~Tope}
\author[11]{A.~Topkar}
\author[25]{F.~R.~Torres}
\author[108]{M.~Torti}
\author[135]{M.~Tortola}
\author[26]{F.~Tortorici}
\author[84]{M.~Toups}
\author[77]{C.~Touramanis}
\author[20]{M.~Tripathi}
\author[43]{I.~Tropin}
\author[65]{W.~H.~Trzaska}
\author[115]{Y.~Tsai}
\author[75]{K.~V.~Tsang}
\author[119]{R.~Tsenov}
\author[143]{S.~Tufanli}
\author[75]{C.~Tull}
\author[41]{J.~Turner}
\author[80]{M.~Tzanov}
\author[8]{E.~Tziaferi}
\author[59]{Y.~Uchida}
\author[61]{J.~Urheim}
\author[115]{T.~Usher}
\author[67]{M.~R.~Vagins}
\author[140]{P.~Vahle}
\author[4]{G.~A.~Valdiviesso}
\author[43]{L.~Valerio}
\author[126]{Z.~Vallari}
\author[135]{J.~Valle}
\author[109]{R.~Van~Berg}
\author[79]{R.~Van~de~Water}
\author[7]{P.~Van~Gemmeren}
\author[106]{F.~Varanini}
\author[48]{G.~Varner}
\author[117]{G.~Vasseur}
\author[43]{K.~Vaziri}
\author[43]{G.~Velev}
\author[106]{S.~Ventura}
\author[17]{A.~Verdugo}
\author[146]{T.~Viant}
\author[25]{T.~V.~Vieira}
\author[73]{C.~Vignoli}
\author[65]{S.~Vihonen}
\author[126]{C.~Vilela}
\author[14]{B.~Viren}
\author[36]{T.~Vrba}
\author[71]{T.~Wachala}
\author[141]{D.~Wahl}
\author[118]{M.~Wallbank}
\author[20]{N.~Walsh}
\author[125]{B.~Wang}
\author[22]{H.~Wang}
\author[121]{L.~Wang}
\author[41]{T.~Wang}
\author[118]{T.K.~Warburton}
\author[33]{D.~Warner}
\author[59]{M.~Wascko}
\author[78]{D.~Waters}
\author[116]{A.~Weber}
\author[12]{M.~Weber}
\author[121]{W.~Wei}
\author[62]{A.~Weinstein}
\author[122]{D.~Wells}
\author[141]{D.~Wenman}
\author[62]{M.~Wetstein}
\author[130]{A.~White}
\author[49]{L.~Whitehead}
\author[61]{D.~Whittington}
\author[126]{M.~Wilking}
\author[43]{J.~Willhite}
\author[43]{P.~Wilson}
\author[33]{R.~J.~Wilson}
\author[84]{L.~Winslow}
\author[35]{P.~Wittich}
\author[19]{H.~H.~Wong}
\author[84]{T.~Wongjirad}
\author[120]{K.~Wood}
\author[14]{E.~Worcester}
\author[14]{M.~Worcester}
\author[146]{S.~Wu}
\author[62]{T.~Xin}
\author[126]{C.~Yanagisawa}
\author[29]{S.~Yang}
\author[43]{T.~Yang}
\author[125]{J.~Ye}
\author[14]{M.~Yeh}
\author[56]{N.~Yershov}
\author[43]{K.~Yonehara}
\author[14]{B.~Yu}
\author[130]{J.~Yu}
\author[15]{J.~Zalesak}
\author[71]{A.~Zalewska}
\author[127]{B.~Zamorano}
\author[118]{L.~Zang}
\author[108]{A.~Zani}
\author[16]{A.~Zani}
\author[46]{G.~Zavala}
\author[43]{G.~Zeller}
\author[14]{C.~Zhang}
\author[121]{C.~Zhang}
\author[32]{E.~D.~Zimmerman}
\author[117]{M.~Zito}
\author[15]{J.~Zuklin}
\author[43]{R.~Zwaska}



\affil[1]{ABC Federal University, Santo Andr\'e \textendash SP, 09210-580, Brazil}

\affil[2]{APC-Paris, Batiment Condorcet;
10, rue Alice Domon et L'eonie Duquet;
F-75205 Paris CEDEX 13, France}

\affil[3]{University of Alabama (Tuscaloosa), Tuscaloosa, AL 35487-0324, USA}

\affil[4]{Federal University of Alfenas at Po\c cos de Caldas, 11999, CEP 37715-900 Po\c cos de Caldas-MG, Brazil}

\affil[5]{Aligarh Muslim University, Department of Physics
Aligarh-202002, India}

\affil[6]{Antananarivo, Pr\'esidence de l'Universit\'e d'Antananarivo: BP 566, Antananarivo 101, Madagascar}

\affil[7]{Argonne National Lab., Argonne, IL 60439, USA}

\affil[8]{University of Athens, University Campus, Zografou  GR 157 84
Greece, Greece}

\affil[9]{Universidad del Atlantico, Km 7 antigua vi  a Puerto Colombia, Barranquilla, Colombia}

\affil[10]{Banaras Hindu University, Varanasi 221 005, India, India}

\affil[11]{Bhabha Atmoic Research Center, Trombay, Mumbai, India}

\affil[12]{University of Bern, Lab for High Energy Physics;
Sidlerstrasse 5; CH-3012 Bern, Switzerland}

\affil[13]{Boston University, Boston, MA 02215, USA}

\affil[14]{Brookhaven National Lab., Upton, NY 11973-5000, USA}

\affil[15]{Institute of Physics CAS, v.v.i.  , Na Slovance 2; 182 21 Praha 8, Czech Republic}

\affil[16]{CERN, European Organization for Nuclear Research
European Laboratory for Particle Physics; 1211 Gen`eve 23, Switzerland}

\affil[17]{CIEMAT, Divisi\'on de F\'{i}sica de Part\'{i}culas; Avenida Complutense 40; E-28040 Madrid, Spain}

\affil[18]{CNR Pisa, 1, 56124 Pisa PI, Italy}

\affil[19]{University of California (Berkeley), \#7300;
Berkeley, CA 94720-7300, USA}

\affil[20]{University of California (Davis), Davis, CA 95616, USA}

\affil[21]{University of California (Irvine), Irvine, CA 92697-4575, USA}

\affil[22]{University of California (Los Angeles), Los Angeles, CA 90095-1547, USA}

\affil[23]{California Institute of Technology, MC 356-48;
Pasadena, CA 91125, USA}

\affil[24]{University of Cambridge, JJ Thomson Avenue, Cambridge CB3 0HE, UK}

\affil[25]{University de Campinas, Av. S\'ergio Buarque de Holanda, 777 CEP 13083-859 Campinas-SP, Brazil}

\affil[26]{University di Catania, Via Santa Sofia, I-95123 Catania, Italy}

\affil[27]{Institute of Particle and Nuclear Physics of the Faculty of Mathematics and Physics of the Charles University in Prague, V Hole\v sovi\v ck\'ach 747/2; 180 00 Praha 8-Libe\v n, Czech Republic}

\affil[28]{University of Chicago, Chicago, IL 60637-1434, USA}

\affil[29]{University of Cincinnati, Cincinnati, OH 45221-0011, USA}

\affil[30]{Cinvestav, 07360 Ciudad de M\'exico, D.F., Mexico}

\affil[31]{Universidad de Colima, Facultad de Ciencias
Bernal Diaz del Castillo 340
Colonia Villa San Sebastian
Colima, Colima, Mexico}

\affil[32]{University of Colorado, Boulder, CO 80309, USA}

\affil[33]{Colorado State University, Fort Collins, CO 80523, USA}

\affil[34]{Columbia University, New York, NY 10027, USA}

\affil[35]{Cornell University, Laboratory for Elementary-Particle Physics; Newman Lab;
Ithaca, NY 14853\textendash5001, USA}

\affil[36]{Czech Technical University in Prague, Brehova 7; 115 19 Praha 1, Czech Republic}

\affil[37]{Dakota State University, Madison, SD 57042, USA}

\affil[38]{University of Delhi, Department of Physics and Astrophysics, Delhi 110007, India}

\affil[39]{Drexel University, Philadelphia, PA 19104, USA}

\affil[40]{Duke University, Durham, NC 27706, USA}

\affil[41]{University of Durham, Institute for Particle Physics Phenomenology;
Dept. of Physics, Ogden Centre for Fund. Physics;
South Road; Durham DH1 3LE, UK}

\affil[42]{University Estadual de Feira de Santana, S/N;44036-900, Feira de Santana-BA, Brazil}

\affil[43]{Fermi National Accelerator Lab, Batavia, IL 60510-0500, USA}

\affil[44]{University Federal de Goias, Goiania, GO, Brazil}

\affil[45]{Gran Sasso Science Institute, 7, L'Aquila, Italy}

\affil[46]{Universidad de Guanajuato, Gto., C.P.37000, Mexico}

\affil[47]{Harish-Chandra Research Institute, Jhunsi, Allahabad 211 019, India}

\affil[48]{University of Hawaii, Honolulu, HI 96822-2219, USA}

\affil[49]{University of Houston, Houston, TX 77204, USA}

\affil[50]{Huddersfield, Huddersfield, West Yorkshire HD1 3DH, UK}

\affil[51]{Horia Hulubei National Institute of Physiscs and Nuclear Engineering, Horia Hulubei National Institute of Physiscs and Nuclear
Engineering, Bucharest-Magurele, Romania}

\affil[52]{University of  Hyderabad, Gachibowli, Hyderabad - 500 046, India}

\affil[53]{Institut de F\`\i{}sica d'Altes Energies (IFAE); Campus Universitat Autonoma de Barcelona , E-08193  Cerdanyola del Valles (Barcelona), Spain}

\affil[54]{Illinois Institute of Technology , Room 182LS; Chicago, IL 60616, USA}

\affil[55]{IIT Hyderabad, Kandi, Hyderabad - 502205, India}

\affil[56]{Institute for Nuclear Research of the Russian Academy of Sciences (INR RAS), 60th October Anniversary Prosp. 7a
Moscow, Russia 117312, Russia}

\affil[57]{Institute for Research in Fundamental Sciences (IPM), Tehran, Iran.
Postal code: 19538-33511
PO Box: 19395-5531, Iran}

\affil[58]{Idaho State University, Department of Physics
921 South 8th Ave.
Stop 8106
Pocatello, ID 83209-8106, USA}

\affil[59]{Imperial College of Science Tech. \& Medicine, Blackett Lab.; Prince Consort Road; London SW7 2BZ, UK}

\affil[60]{Indian Institute of Technology Guwahati, Guwahati, 781 039, India}

\affil[61]{Indiana University, Bloomington, IN 47405-7105, USA}

\affil[62]{Iowa State University, Ames, IA 50011, USA}

\affil[63]{Institut de Physique Nucleaire de Lyon (IPNL), Rue E. Fermi 4
69622 Villeurbanne, France}

\affil[64]{University of Jammu, Physics Department, JAMMU-180006, India}

\affil[65]{University of Jyvaskyla, FI-40014, University of Jyvaskyla, Finland}

\affil[66]{Kansas State University, Manhattan, KS 66506, USA}

\affil[67]{Kavli Institute for the Physics and Mathematics of the Universe (WPI), Kashiwa, Chiba 277-8582, Japan}

\affil[68]{KEK, High Energy Accelerator Research Organization
1\textendash1 Oho, Tsukuba-shi; Ibaraki-ken 305-0801, Japan}

\affil[69]{KYIV National University, Department of Nuclear Physics, 64, 01601 Kyiv, Ukraine}

\affil[70]{Koneru Lakshmaiah, , India}

\affil[71]{Krakow, Go\l{}ebia 24, 31-007 Krak\'ow, Poland}

\affil[72]{Lab. d'Annecy-le-Vieux de Phys. des Particules, BP 110; F-74941 Annecy-le-Vieux CEDEX, France}

\affil[73]{Laboratori Nazionali del Gran Sasso, I-67010 Assergi, AQ, Italy}

\affil[74]{Lancaster University, Bailrigg, Lancaster LA1 4YB, UK}

\affil[75]{Lawrence Berkeley National Lab., Berkeley, CA 94720-8153, USA}

\affil[76]{Universit\'e de Li\`ege, Bat B5, Sart Tilman B-4000, Belgium}

\affil[77]{University of Liverpool, L69 7ZE, Liverpool, UK}

\affil[78]{University College London, London, WC1E 6BT, UK}

\affil[79]{Los Alamos National Laboratory, Los Alamos, NM 87545, USA}

\affil[80]{Louisiana State University, Baton Rouge, LA 70803-4001, USA}

\affil[81]{University of Lucknow, Department of Physics
Lucknow 226007
Uttar Pradesh, India}

\affil[82]{University of Manchester, Oxford Road, Manchester M13 9PL, UK}

\affil[83]{University of Maryland, College Park, MD 20742-4111, USA}

\affil[84]{Massachusetts Institute of Technology, Cambridge, MA 02139-4307, USA}

\affil[85]{University of Puerto Rico, Box 9016; Mayaguez, PR 00681-9000, USA}

\affil[86]{University of Michigan, Ann Arbor, MI 48109-1040, USA}

\affil[87]{Michigan State University, East Lansing, MI 48824, USA}

\affil[88]{University di Milano, INFN Sezione di Milano, I-20133 Milano, Italy}

\affil[89]{INFN Sezione di Milano Bicocca, Piazza della Scienza 3, 20126 Milano, Italy}

\affil[90]{University of Minnesota (Twin Cities), Minneapolis, MN 55455, USA}

\affil[91]{University of Minnesota (Duluth), Duluth, MN 55812, USA}

\affil[92]{NIKHEF, Science Park, Amsterdam, Netherlands}

\affil[93]{Istituto Nazionale di Fisica Nucleare - Sezione di Napoli, Complesso Universitario di Monte S. Angelo, I-80126 Napoli, Italy}

\affil[94]{National Centre for Nuclear Research, A. Soltana 7, 05 400 Otwock, Poland}

\affil[95]{Jawaharlal Nehru University, New Delhi 110067, INDIA, India}

\affil[96]{University of New Mexico, MSC07 4220;
Albuquerque, NM 87131, USA}

\affil[97]{Northwestern University, Evanston, Il 60208, USA}

\affil[98]{University of Notre Dame, Notre Dame, IN 46556-5670, USA}

\affil[99]{Observatorio Nacional, Vassouras - RJ, 27700-000, Brazil}

\affil[100]{Ohio State University, Dept. of Physics; 191 W. Woodruff Ave.;
Columbus, OH 43210, USA}

\affil[101]{Oregon State University, Dept. of Physics;
301 Weniger Hall; Corvallis, OR 97331\textendash6507, USA}

\affil[102]{University of Oxford, Oxford, OX1 3RH, UK}

\affil[103]{Pacific Northwest National Lab, , USA}

\affil[104]{Pennsylvania State University, PMB 264;
University Park, PA 16802-6300, USA}

\affil[105]{PUCP, Av. Universitaria 1801, Lima, Peru}

\affil[106]{University of Padova, Dip. Fisica e Astronomia G. Galilei and INFN Sezione di
Padova, I-35131 Padova, Italy}

\affil[107]{Panjab University, Chandigarh, 160014 U.T., India}

\affil[108]{University of Pavia, INFN Sezione di Pavia, I-27100 Pavia, Italy}

\affil[109]{University of Pennsylvania, Philadelphia, PA 19104-6396, USA}

\affil[110]{University di Pisa, Theor. Division;
Largo B. Pontecorvo 3, Ed. B-C; I-56127 Pisa, Italy}

\affil[111]{University of Pittsburgh, Pittsburgh, PA 15260, USA}

\affil[112]{Princeton University, Princeton, New Jersey 08544-0708, USA}

\affil[113]{Punjab Agri. University, Centre for High Energy Physics;
Lahore - 54590, India}

\affil[114]{University of Rochester, Rochester, NY 14627-0171, USA}

\affil[115]{SLAC National Acceleratory Laboratory, Menlo Park, CA 94025, USA}

\affil[116]{STFC Rutherford Appleton Laboratory, Harwell Oxford, Didcot OX11 0QX, UK}

\affil[117]{CEA/Saclay, IPhT; Inst. de Physique Theorique;
Orme des Merisiers, Point Courrier 136;
F-91191 Gif-sur-Yvette CEDE, France}

\affil[118]{University of Sheffield, Sheffield, S3 7RH, UK}

\affil[119]{University of Sofia, Atomic Physics Dept., Faculty of Physics;
5 James Bourchier Blvd.; BG-1164 Sofia, Bulgaria}

\affil[120]{University of South Carolina, Columbia, SC 29208, USA}

\affil[121]{University of South Dakota, Vermillion, SD 57069, USA}

\affil[122]{South Dakota School of Mines and Technology, Rapid City, SD 57701, USA}

\affil[123]{South Dakota Science And Technology Authority, Lead, SD 57754, USA}

\affil[124]{South Dakota State University, Brookings, SD 57007, USA}

\affil[125]{Southern Methodist University, Dallas, TX 75275, USA}

\affil[126]{Stony Brook University, Nucleon Decay and Neutrino Physics Group
Department of Physics and Astronomy
Stony Brook University
Stony Brook, NY 11794-3800, USA}

\affil[127]{University of Sussex, Brighton, BN1 9RH, UK}

\affil[128]{Syracuse University, Syracuse, NY 13244-1130, USA}

\affil[129]{University of Tennessee at Knoxville, Knoxville, TN, USA}

\affil[130]{University of Texas (Arlington), Arlington, TX 76019, USA}

\affil[131]{University of Texas (Austin), Austin, TX 78712-0264, USA}

\affil[132]{TUBITAK Space Technologies Research Institute , TR-06800, Ankara, Turkey}

\affil[133]{Tufts University, Medford, MA 02155, USA}

\affil[134]{Variable Energy Cyclotron Centr, 1/AF, Bidhannagar
Kolkata - 700 064
West Bengal, India}

\affil[135]{Instituto de Fisica Corpuscular, C/Catedratico Jose Beltran, 2
E-46980 Paterna (Valencia), Spain}

\affil[136]{Virginia Tech., Blacksburg, VA 24061-0435, USA}

\affil[137]{University of Warsaw, Faculty of Physics 
ul. Pasteura 5
02-093 Warsaw, Poland}

\affil[138]{Univ. of Warwick, Coventry CV4 7AL, UK}

\affil[139]{Wichita State University, Physics Division
1845 Fairmount St.
Wichita, KS 67260-0032, USA}

\affil[140]{College of William and Mary, Williamsburg, VA 23187-8795, USA}

\affil[141]{University of Wisconsin, Madison, WI 53706, USA}

\affil[142]{Wroclaw University, Plac Maxa Borna 9, 50-204 Wroclaw, Poland}

\affil[143]{Yale University, New Haven, CT 06520, USA}

\affil[144]{Yerevan Institute for Theoretical Physics and Modeling, Halabian Str. 34; Yerevan 0036, Armenia}

\affil[145]{York, Physics and Astronomy Dept.;
4700 Keele St.; Toronto M3J 1P3, Canada}

\affil[146]{ETH Zurich, HPK F 23
Schafmattstr. 20
8093 Z\"urich, Switzerland}




==> bibliography.tex <==
\begin{thebibliography}{99}
\end{thebibliography}


==> calibration_strategy.tex <==

\section{Calibration Strategy}
%\fixme{from Josh K}
%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{Motivation}


	The scientific program of protoDUNE is critical to the ultimate success
of DUNE.  ProtoDUNE will be the DUNE Collaboration's only opportunity to
measure the response of a DUNE-style LAr-TPC to hadrons (as well as $\gamma$s,
$\mu$s, and electrons), and to compare those measurements to a model of the
detector response. That model can then be used to predict the response for DUNE
itself.  Precision measurements of response in testbeams are a common approach
of long-baseline neutrino experiments. As a recent example, NO{$\nu$}A has
found that some of their measurements are limited by the lack of knowledge of
this response, which a testbeam would have provided.
	
	By itself, however, protoDUNE does {\it not} provide a response
measurement that can simply be mapped onto DUNE.  Rather, protoDUNE provides
measurements of the part of the response that depends on the interactions of
various particle species in LAr.  The remainder of the detector response, which
includes reconstruction resolutions and biases, the effects of noise, space
charge and how it impacts reconstruction, and the conversion from observed
charge to energy, all must be calibrated and ultimately removed from the
physical hadron response.  Misinterpreting, for example, longitudinal diffusion
as a fundamental part of shower development of $\pi^+$s means our understanding
of $\pi$s will be wrong in DUNE---and there will be no test of that response in
the DUNE FD, independent of neutrino events themselves.  By building protoDUNE
in a way that mimics the DUNE far detector, one would still have to assume that such errors will
`cancel out';
 in practice one cannot rely on such a cancellation without knowing
how different the parameters governing the response may be.

	Ultimately, what this means is that one must calibrate a model of the
detector---likely a LArSoft model---and use it to predict the response to
hadrons.  If the detector model is accurate, differences between the predicted
response to various hadrons and measurements allows a correction to the hadron
response that can be used for the DUNE experiment.  

	The existing option for creating a calibrated detector model for
protoDUNE is to presume that calculations of the electric field throughout the
detector, including space charge effects and impurities, are accurate, and that
with this as input the detector response is uniquely calculable throughout the
volume and for all times, up to the details of the electronics transfer
function (and of course the response to various particle species which is what
is being measured by protoDUNE).  

	Figure~\ref{fig:35t} shows the variations in electron lifetime within
\fixme{where is figure in this doc ?}
the 35 tonne prototype as a function of position, as measured by {\it in-situ}
purity monitors. The clear differences top and bottom indicate that we cannot
assume that measurements in just a few places represent the detector as a
whole. In addition to these variations, changes with the ambient environment
were also seen, indicating that measurements must be made with reasonable
frequency as well.  An idealized view of how an operating detector will behave
would miss such variations.
	 
	        The calibration program for DUNE has as its goal both the
measurement of the parameters governing detector response and {\it tests} of
the predicted response.  Table~\ref{tbl:params} lists many of the critical
%
\begin{table}
\begin{center}
\begin{tabular}{|l| l| l| l| l| } \hline \hline
{\bf Parameter} & {\bf Name} & {\bf Ex-situ Calibration} & {\bf Calibration} & {\bf Test} \\ \hline
$W$ & Ionization Energy  & Benchtop & None & Cosmics \\
$C$ & ADC/Charge Map & Benchtop Pulsers & Front-End Pulsers & Stopped cosmics \\
$f$ & Energy Scale & Calculation & Stopped cosmics & Through-going cos. \\
$R$ & Electron recombination & Calculation & Through-going cosmics & Michels\\
$\tau$ & Electron lifetime & Purity Monitors & Through-going cosmics & Stopped
cosmics\\
$\vec{E}(\vec{r})$ & Electric Field map & Calculation & Crossing cosmics/halo &
Michels \\
$v_d$ & Drift Speed & Purity+temp+Calc.& triggered cosmics & None \\
$d$ & Electron Diffusion & Calculation & triggered cosmics & None \\
$\rho_E$ & Field response & Calculation & Through-going cosmics & None \\ \hline \hline
\end{tabular}
\caption{Parameters to be calibrated for ProtoDUNE model\label{tbl:params}}
\end{center}
\end{table}
%
parameters that need to be measured, and what will be available in protoDUNE
for both measurements of the parameters and tests of the resulting calibrated
model.  Unfortunately, time and budget constraints will prevent us from
building and deploying a laser system like that used in other surface
single-phase LAr-TPCs.  ProtoDUNE calibrations will rely solely on cosmic rays---those triggered by
going through a set of external tracking scintillation panels.  
%ProtoDUNE will
%be the first large-scale, surface single-phase LAr-TPC to make physics
%measurements using only calibrations from cosmic rays, and will therefore
%represent a triumph of the DUNE ``no LAr-TPC calibration device needed''
%philosophy.
%%% --- I like this sentence but it may be better not to trigger those kinds of discussions with the SPSC reviewers - TK ---

It is assumed that there will be
several auxiliary systems that already provide measurements or estimates of
some of these parameters:
\begin{itemize}
\item Monitors of HV and current to the APAs \fixme{verify whether this is the case}
\item Survey of wire positions \fixme{verify whether this is planned}
\item Temperature sensors {\it in situ} at several places in the volume
\item Purity monitors at several positions within the volume
\item Front-end electronics response calibration pulsers.
\end{itemize}
        These systems provide the initial input to the model for electric
field, and for calculations of average drift velocity, electron lifetime, and
electron diffusion.  The goal of the calibration system described here 
is first to measure the response parameters with granularity in time and
position that cannot be accomplished by the above systems, and to test the
resultant model with tracks of known positions, trajectories, and energy
deposits.


\fixme{xxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxxx}
The planned cosmic muon tagging hardware is described in section \ref{sec:muontagger}

        Although there are many possible configurations for deployment of the
counters, a particularly interesting deployment would be fore-and-aft,
therefore triggering on muons that had trajectories similar to beam events. In
this configuration, the counters could also serve as a tagger for beam halo
events.  By tagging such events, only those whose energy and position are
reasonably well constrained will be part of the beam calibration.

        To fully measure the field map using cosmic rays, crossing
tracks to resolve ambiguities in the field direction are needed.  Our studies have shown
that even with counters just fore-and-aft, we can illuminate the detector
using halo muons that pass through both counters (i.e., roughly horizontally)
that cross cosmic tracks going through just one counter. In this case, the
trajectory of the cosmic ray inside the TPC is determined by the TPC itself.
While this argument appears problematic since it is the TPC we are attempting
to calibrate in the first place, we anticipate that the longitudinal field is
known well enough, even in the presence of large space charge effects, that
uncertainties in the drift velocity will be small.  While this has not yet been
quantitatively demonstrated in a real large-scale detector, for ProtoDUNE the plan 
is to use cosmics that go through both sets of counters to determine the drift
velocity field map (independently of determination of the electric field map)
and to use that map (rather than the electric field map) to reconstruct the
crossing tracks.  The collaboration has not yet explored whether the correlation between
these two approaches will lead to an unacceptably large uncertainty on the
field.

 While the fore-aft deployment scheme works well for calibration plans,
it provides little help on tagging cosmics that could cause difficulty for
reconstruction algorithms, since the vast majority of those will be
downward-going.  Reconstruction, however, has progressed significantly and
there is no expectation that existing algorithms will have problems identifying
beam-related tracks and showers beneath the rain of cosmics. There is therefore
no need for counters above and below the detector.

        In addition to using the triggered horizontal cosmics to measure the
drift velocity map, and the crossing halo muons with high-angle cosmics to
determine the transverse field components, we will also use stopped cosmics to
provide a measure of the detector's energy scale. Stopped cosmics have the
advantage that about a meter upstream of the track endpoint the muon is a MIP
and dE/dx is very well known. The techniques of using these has been
demonstrated very successfully in both MINOS and NOvA, and MicroBooNE has made
excellent progress in using these as a calibration as well. Once stopped cosmics have been 
used as a calibration source, the quality of the calibration can be tested by looking at the Michel
spectrum (using the same stopped events) and ultimately the mass peak of
reconstructed $\pi^0$s produced from charged pion beam events.


%%%%%%%%%%%%%%%%%%%%%%%%%%
%%\subsubsection{PDS Calibration Run Plan}
 %%    Run/Measurement plan  -- Toups ?
  %%   Light yield vs. field
   %%  timing studies,
   %%  beam off trigger



==> common/acronyms-shared-vol1-2-4.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%% COMMON list for acronyms below %%%%%%%%%%%%%%%
\nomenclature{$\mathcal{O}(n)$}{of order $n$}
\nomenclature{3D}{3 dimensional (also 1D, 2D, etc.)} % not phys
\nomenclature{CDR}{Conceptual Design Report}
\nomenclature{CF}{Conventional Facilities}
\nomenclature{CP}{product of charge and parity transformations}
\nomenclature{CPT}{product of charge, parity and time-reversal transformations}
\nomenclature{CPV}{violation of charge and parity symmetry}
\nomenclature{DAQ}{data acquisition}
\nomenclature{DOE}{U.S. Department of Energy}
\nomenclature{DUNE}{Deep Underground Neutrino Experiment}
\nomenclature{ESH}{Environment, Safety and Health}
\nomenclature{eV}{electron volt, unit of energy (also keV, MeV, GeV, etc.)}
\nomenclature{FD}{far detector}
\nomenclature{FGT}{Fine-Grained Tracker}
\nomenclature{FSCF}{far site conventional facilities}
\nomenclature{NSCF}{near site conventional facilities}
\nomenclature{GUT}{grand unified theory}
\nomenclature{\ktyr}{exposure (without beam), expressed in kilotonnes times years}
\nomenclature{\ktMWyr}{exposure, expressed in kilotonnes $\times$ megawatts $\times$ years, based on 56\% beam uptime and efficiency} 
\nomenclature{L}{level, indicates depth in feet underground at the far site, e.g., 4850L}
\nomenclature{LAr}{liquid argon}
\nomenclature{LArTPC}{liquid argon time-projection chamber}
\nomenclature{LBL}{long-baseline (physics)}
\nomenclature{LBNF}{Long-Baseline Neutrino Facility}
\nomenclature{MH}{mass hierarchy}
\nomenclature{MI}{Main Injector (at Fermilab)}
\nomenclature{ND}{near neutrino detector}
\nomenclature{NDS}{Near Detector Systems; refers to the collection of detector systems at the near site }
\nomenclature{near detector}{except in Volume 4 Chapter 7, \textit{near detector} refers to the \textit{neutrino} detector system in the NDS}
\nomenclature{POT}{protons on target}
\nomenclature{QA}{quality assurance}
\nomenclature{SM}{Standard Model of particle physics}
\nomenclature{t}{metric ton, written \textit{tonne} (also kt)}
\nomenclature{tonne}{metric ton}
\nomenclature{TPC}{time-projection chamber (not used as `total project cost' in the CDR)}


==> common/acronyms-shared-vol1-2.tex <==
%%%%%%%%%%%%% PROJECT AND PHYSICS VOLUME list for acronyms below %%%%%%%%%%%%
\nomenclature{CKM}{(CKM matrix) Cabibbo-Kobayashi-Maskawa matrix, also known as
quark mixing matrix} 
\nomenclature{C.L.}{confidence level}
\nomenclature{octant}{any of the eight parts into which 4$\pi$ is divided by three mutually perpendicular axes; the range of the PMNS angles is $0$ to $\pi/2$, which spans only two of the eight octants}
\nomenclature{PMNS}{(PMNS matrix) Pontecorvo-Maki-Nakagawa-Sakata matrix, also known as
the lepton or neutrino mixing matrix} 


==> common/acronyms-shared-vol1-4.tex <==
%%%%%%%%%%%%% PROJECT AND DETECTORS VOLUME list for acronyms below %%%%%%%%%%%%

\nomenclature{APA}{anode plane assembly} 
\nomenclature{BLM}{(in Volume 4) beamline measurement (system); (in Volume 3) beam loss monitor}
\nomenclature{CPA}{cathode plane assembly}
\nomenclature{ECAL}{electromagnetic calorimeter}
\nomenclature{GAr}{gaseous argon}
\nomenclature{HV}{high voltage}


==> common/acronyms-shared-vol2-4.tex <==
%%%%%%%%%%%%% PHYSICS AND DETECTORS VOLUME list for acronyms below %%%%%%%%%%%%
\nomenclature{CC}{charged current (interaction)}
\nomenclature{DIS}{deep inelastic scattering}
\nomenclature{FSI}{final-state interactions}
\nomenclature{GEANT4}{GEometry ANd Tracking, a platform for the simulation of the passage of particles through matter using Monte Carlo methods} 
\nomenclature{GENIE}{Generates Events for Neutrino Interaction Experiments (an object-oriented neutrino Monte Carlo generator)} 
\nomenclature{MC}{Monte Carlo (detector simulation methods)}
\nomenclature{QE}{quasi-elastic (interaction)}

==> common/acronyms-vol1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%% PROJECT VOLUME list for acronyms below %%%%%%%%%%%%%%%
\nomenclature{L1, L2, ...}{WBS level within the LBNF and DUNE Projects, where the overall Project is L1}
\nomenclature{MOU}{memorandum of understanding}
\nomenclature{PIP-II(III)}{Proton Improvement Plan (II or III)}
\nomenclature{SDSTA}{South Dakota Science and Technology Authority}
\nomenclature{WBS}{Work Breakdown Structure}


==> common/acronyms-vol2.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%% PHYSICS VOLUME list for acronyms below %%%%%%%%%%%%%%%
\nomenclature{BR}{branching ratio}
\nomenclature{DM}{dark matter}
\nomenclature{DSNB}{Diffuse Supernova Neutrino Background}
\nomenclature{ENC}{???}
\nomenclature{GLoBES}{General Long-Baseline Experiment Simulator (software package)}
\nomenclature{L/E}{length-to-energy ratio}
\nomenclature{LRI}{long-range interactions}
\nomenclature{$M_{\odot}$}{solar mass}
\nomenclature{NC}{neutral current (interaction)}
\nomenclature{NH}{normal (mass) hierarchy}
\nomenclature{NSI}{nonstandard interactions}
\nomenclature{MSW}{Mikheyev-Smirnov-Wolfenstein (effect)}
\nomenclature{SME}{Standard-Model Extension}
\nomenclature{SUSY}{supersymmetry}
\nomenclature{WIMP}{weakly-interacting massive particle}


==> common/acronyms-vol4.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%% DETECTORS VOLUME list for acronyms below %%%%%%%%%%%%%%%

\nomenclature{CE}{Cold Electronics}
\nomenclature{COB}{cluster on-board (motherboards)} %?
\nomenclature{CRP}{Charge-Readout Planes }
\nomenclature{DRAM}{dynamic random access memory}
\nomenclature{FE}{front end (electronics)}
%\nomenclature{Fermilab (also FNAL)}{Fermi National Accelerator Laboratory (in Batavia, IL, the Near Site)}
%\nomenclature{FNAL}{see Fermilab}
\nomenclature{FPGA}{field programmable gate array} %?
\nomenclature{FGT}{Fine-Grained Tracker}
\nomenclature{FS}{full stream (data volumes)} %?
\nomenclature{LEM}{Large Electron Multiplier}
\nomenclature{LNG}{liquefied natural gas}
%\nomenclature{LNGS}{Laboratori Nazionali (National Laboratory) del Gran Sasso (in L'Aquila, Italy)}
%\nomenclature{MaVaNs}{mass varying neutrinos}
\nomenclature{MIP}{minimum ionizing particle}
\nomenclature{MTS}{Materials Test Stand}
\nomenclature{MuID}{muon identifier (detector)}
%\nomenclature{OPERA}{Oscillation Project with Emulsion-Racking Apparatus (experiment at LNGS)}
\nomenclature{NND}{(used only in Volume 4 Chapter 7) near neutrino detector, same as ND}
%\nomenclature{OD}{outer diameter}
\nomenclature{PD}{photon detection (system)}
\nomenclature{PMT}{photomultiplier tube}
\nomenclature{PPM/PPB/PPT}{parts per million/billion/trillion}
\nomenclature{RCE}{reconfigurable computing element}
\nomenclature{RIO}{reconfigurable input output}
\nomenclature{RPC}{resistive plate chamber}
\nomenclature{SiPM}{silicon photomultiplier}
\nomenclature{S/N}{signal-to-noise (ratio)}
\nomenclature{SSP}{SiPM signal processor}
\nomenclature{SBN}{Short-Baseline Neutrino program (at Fermilab)}
\nomenclature{STT}{straw tube tracker}
%\nomenclature{SURF (also Sanford Lab)}{Sanford Underground Research Facility (in Lead, SD, the Far Site)}
\nomenclature{TR}{transition radiation}
%\nomenclature{W}{Watt (also mW, kW, MW) }
%\nomenclature{WA105}{Single-Phase LArTPC and the Long Baseline Neutrino Observatory Demonstration}
\nomenclature{WLS}{wavelength shifting}
\nomenclature{ZS}{zero suppression}


==> common/acronyms.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%% COMMON list for acronyms below %%%%%%%%%%%%%%%
\nomenclature{$\mathcal{O}(n)$}{of order $n$}
\nomenclature{3D}{3 dimensional (also 1D, 2D, etc.)} % not phys
\nomenclature{CDR}{Conceptual Design Report}
\nomenclature{CF}{Conventional Facilities}
\nomenclature{CP}{product of charge and parity transformations}
\nomenclature{CPT}{product of charge, parity and time-reversal transformations}
\nomenclature{CPV}{violation of charge and parity symmetry}
\nomenclature{DAQ}{data acquisition}
\nomenclature{DOE}{U.S. Department of Energy}
\nomenclature{DUNE}{Deep Underground Neutrino Experiment}
\nomenclature{ESH}{Environment, Safety and Health}
\nomenclature{eV}{electron-Volt, unit of energy (also keV, MeV, GeV, etc.)}
\nomenclature{FD}{far detector}
\nomenclature{FGT}{Fine-Grained Tracker}
\nomenclature{FSCF}{far site conventional facilities}
\nomenclature{NSCF}{near site conventional facilities}
\nomenclature{GUT}{grand unified theory}
\nomenclature{\ktyr}{exposure (without beam), expressed in kilotonnes times years}
\nomenclature{\ktMWyr}{exposure, expressed in kilotonnes $\times$ megawatts $\times$ years} 
\nomenclature{L}{level, indicates depth in feet underground at the far site, e.g., 4850L}
\nomenclature{LAr}{liquid argon}
\nomenclature{LArTPC}{liquid argon time-projection chamber}
\nomenclature{LBL}{long-baseline (physics)}
\nomenclature{LBNF}{Long-Baseline Neutrino Facility}
\nomenclature{MH}{mass hierarchy}
\nomenclature{MI}{Main Injector (at Fermilab)}
\nomenclature{ND}{near neutrino detector}
\nomenclature{NDS}{Near Detector Systems; refers to the collection of detector systems at the near site }
\nomenclature{near detector}{except in Volume 4 Chapter 7, this refers to the \textit{neutrino} detector system in the NDS}
\nomenclature{NND}{(used only in Volume 4 Chapter 7) near neutrino detector, same as ND}
\nomenclature{POT}{protons on target}
\nomenclature{QA}{quality assurance}
\nomenclature{SM}{Standard Model of particle physics}
\nomenclature{t}{metric ton, written \textit{tonne} (also kt)}
\nomenclature{TPC}{time-projection chamber (not used as `total project cost' in the CDR)}

%%%%%%%%%%%%%%%%%%%%%%%%% PROJECT VOLUME list for acronyms below %%%%%%%%%%%%%%%
\nomenclature{L1, L2, ...}{WBS level within the LBNF and DUNE Projects, where the overall Project is L1}
\nomenclature{MOU}{memorandum of understanding}
\nomenclature{SDSTA}{South Dakota Science and Technology Authority}
\nomenclature{WBS}{Work Breakdown Structure}


%%%%%%%%%%%%%%%%%%%%%%%%% PHYSICS VOLUME list for acronyms below %%%%%%%%%%%%%%%
\nomenclature{BR}{branching ratio}
\nomenclature{DM}{dark matter}
\nomenclature{DSNB}{Diffuse Supernova Neutrino Background}
\nomenclature{GLoBES}{General Long-Baseline Experiment Simulator (software package)}
\nomenclature{L/E}{length-to-energy ratio}
\nomenclature{LRI}{long-range interactions}
\nomenclature{$M_{\odot}$}{solar mass}
\nomenclature{NC}{neutral current (interaction)}
\nomenclature{NH}{normal (mass) hierarchy}
\nomenclature{NSI}{nonstandard interactions}
\nomenclature{MSW}{Mikheyev-Smirnov-Wolfenstein (effect)}
\nomenclature{SME}{Standard-Model Extension}
\nomenclature{SUSY}{supersymmetry}
\nomenclature{WIMP}{weakly-interacting massive particle}

%%%%%%%%%%%%% PROJECT AND PHYSICS VOLUME list for acronyms below %%%%%%%%%%%%
\nomenclature{C.L.}{confidence level}

%%%%%%%%%%%%% PROJECT AND DETECTORS VOLUME list for acronyms below %%%%%%%%%%%%

\nomenclature{APA}{anode plane assembly} 
\nomenclature{BLM}{(in Volume 4) beamline measurement (system); (in Volume 3) beam loss monitor}
\nomenclature{CPA}{cathode plane assembly}
\nomenclature{ECAL}{electromagnetic calorimeter}
\nomenclature{GAr}{gaseous argon}
\nomenclature{HV}{high voltage}

%%%%%%%%%%%%% PHYSICS AND DETECTORS VOLUME list for acronyms below %%%%%%%%%%%%
\nomenclature{CC}{charged current (interaction)}
\nomenclature{DIS}{deep inelastic scattering}
\nomenclature{FSI}{final-state interactions}
\nomenclature{GEANT4}{GEometry ANd Tracking, a platform for the simulation of the passage of particles through matter using Monte Carlo methods} 
\nomenclature{GENIE}{Generates Events for Neutrino Interaction Experiments (an object-oriented neutrino Monte Carlo generator)} 
\nomenclature{MC}{Monte Carlo (detector simulation methods)}
\nomenclature{QE}{quasi-elastic (interaction)}

%%%%%%%%%%%%%%%%%%%%%%%%% DETECTORS VOLUME list for acronyms below %%%%%%%%%%%%%%%

\nomenclature{CE}{Cold Electronics}
\nomenclature{COB}{cluster on-board (motherboards)} %?
\nomenclature{CRP}{Charge-Readout Planes }
\nomenclature{DRAM}{dynamic random access memory}
\nomenclature{FE}{front end (electronics)}
%\nomenclature{Fermilab (also FNAL)}{Fermi National Accelerator Laboratory (in Batavia, IL, the Near Site)}
%\nomenclature{FNAL}{see Fermilab}
\nomenclature{FPGA}{field programmable gate array} %?
\nomenclature{FGT}{Fine-Grained Tracker}
\nomenclature{FS}{full stream (data volumes)} %?
\nomenclature{LEM}{Large Electron Multiplier}
%\nomenclature{LNGS}{Laboratori Nazionali (National Laboratory) del Gran Sasso (in L'Aquila, Italy)}
%\nomenclature{MaVaNs}{mass varying neutrinos}
\nomenclature{MIP}{minimum ionizing particle}
\nomenclature{MTS}{Materials Test Stand}
\nomenclature{MuID}{muon identifier (detector)}
%\nomenclature{OPERA}{Oscillation Project with Emulsion-Racking Apparatus (experiment at LNGS)}
\nomenclature{octant}{any of the eight parts into which 4$\pi$ is divided by three mutually perpendicular axes}
%\nomenclature{OD}{outer diameter}
\nomenclature{PD}{photon detection (system)}
\nomenclature{PMT}{photomultiplier tube}
\nomenclature{RCE}{reconfigurable computing element}
\nomenclature{RIO}{reconfigurable input output}
\nomenclature{RPC}{resistive plate chamber}
\nomenclature{SiPM}{silicon photomultiplier}
\nomenclature{S/N}{signal-to-noise (ratio)}
\nomenclature{SSP}{SiPM signal processor}
\nomenclature{STT}{straw tube tracker}
%\nomenclature{SURF (also Sanford Lab)}{Sanford Underground Research Facility (in Lead, SD, the Far Site)}
\nomenclature{TR}{transition radiation}
%\nomenclature{W}{Watt (also mW, kW, MW) }
%\nomenclature{WA105}{Single-Phase LArTPC and the Long Baseline Neutrino Observatory Demonstration}
\nomenclature{WLS}{wavelength shifting}
\nomenclature{ZS}{zero suppression}

\fixme{Do we need GVKM, SNO, QCD,  PANDORA,  aTCA and microTCA, AMC, MCH, CPU, GPU, VHDL, OpenCL, PTP, Sync-E, GPS, IEEE, WR}







==> compileitprint <==
#!/bin/sh
pdflatex "\def\isfinal{1} \input{$1}"
pdflatex "\def\isfinal{1} \input{$1}"
bibtex $1
pdflatex "\def\isfinal{1} \input{$1}"
pdflatex "\def\isfinal{1} \input{$1}"
makeindex $1.nlo -s nomencl.ist -o $1.nls
pdflatex "\def\isfinal{1} \input{$1}"
pdflatex "\def\isfinal{1} \input{$1}"


==> det-comp-test.tex <==
%\chapter{det-comp}
%This chapter is split into individual files by section



%\input{det-comp/det-comp-overview}
%\input{det-comp/apa}
\input{det-comp/cpa}
%\input{det-comp/field-cage}
%\input{det-comp/hv-comps}
%\input{det-comp/tpc-fe-elec}
%\input{det-comp/pds}
%\input{det-comp/pds-fe-elec-and-daq}
%\input{det-comp/daq}
%\input{det-comp/cryo-feedthroughs}
%%%%%%% moved \input{det-comp/installation}
%\input{det-comp/cryo-lar-purif}
%\input{det-comp/det-mon-slow-ctrl}
%\input{det-comp/calibration} -- leave out per Gina
%\input{det-comp/beam-plug}


==> det-comp/calibration.tex <==


\section{Cosmic muon tagger}
\label{muontagger}

        While there may be motivations from a reconstruction standpoint for a
cosmic veto, from a calibration standpoint a tracking system to provide known 
cosmic trajectories is of interest. The tracker may also be used for
off-beam triggering on stopped muons, as well as detector triggering during
times when there is no beam.

        Counters for a cosmic tracker are available from spares made for the
Double CHOOZ experiment \cite{mucounters}. Light created in the
counters is transmitted via fibers to a 64-anode PMT and read out via
electronics that use a USB interface.  The counter granularity is roughly 2.5~cm, but
multiple layers of the counters could be used for finer granularity.

\fixme{This is a VERY sparse description of a muon tagger system for a TDR. A picture of a 3D model,
amount of area covered, readout and data stream issues would be good to address at least at some level.
Assume some baseline option and mention that changes/"optimizations" are still being considered.}

        Although there are many possible configurations for deployment of the
counters, a particularly interesting deployment would be fore-and-aft,
therefore triggering on muons that had trajectories similar to beam events. In
this configuration, the counters could also serve as a tagger for beam halo
events.  By tagging such events, only those whose energy and position are
reasonably well constrained will be part of the beam calibration.



%%%%%%%%%%%%%%%%%%%%%%%%%%
%%---\subsection{PDS Calibration} -- ANL -- Zelimir
%%---     Mechanical design -- Zelimir interface with Bob Sands?

%%%%%%%%%%%%%%%%%%%%%%%%%%
%%\subsubsection{PDS Calibration Run Plan}
 %%    Run/Measurement plan  -- Toups ?
  %%   Light yield vs. field
   %%  timing studies,
   %%  beam off trigger

%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{QC Procedures}

\fixme{Any QC procedures for the cosmic tagger ??}


==> det-overview.tex <==
%\chapter{det-overview}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Detector Requirements}\label{sec:detector_requirements}

insert detector overview + requirements here \fixme{The whole chapter is `overview'; insert detector requirements here! Link added.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Liquid argon detector properties}
- Electron drift + LAr purity etc.
- LAr scintillation light 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{TPC Signal Formation}\label{sec:tpc_signal_formation}


The principle of a large single-phase LArTPC with wire readout is shown in 
Figure~\ref{fig:signal}. When charged particles traverse the LAr,
ionization electrons are generated. They %would 
travel at a constant speed 
($\sim$1.6 km/s at 500~V/cm electric field) along the electric field 
toward the anode plane assembly (APA) which consists of multiple anode wire planes. 
The first two wire planes encountered collect 
an induction signal as the drifting charges pass through.  The charge is collected 
on the wires of the third plane. The transparency of the induction planes is assured by 
applying appropriate bias voltages to all three wire planes. As charges drift pass the induction 
plane wires and are collected on the anode wires
a current is produced on the wires. Since the locations of all wires are 
accurately known, the position of the ionization charge in the direction 
transverse to the drift can be determined in three independent views. The time 
of the initial interaction can be determined by collecting scintillation light 
in a fast optical detector system. By measuring the time from the light signal 
to electrical signals on the wires, it is possible to determine the longitudinal position 
along the drift direction, leading to %. Therefore, one can achieve 
a 3D image of the trajectories 
of the charged particles in the LAr. The amount of ionization electrons depends on 
the energy and type of the initial particles, and can be used to deduce their properties.

\begin{cdrfigure}[The principles of LArTPC technology]{signal}{The principles of LArTPC technology are shown. (left) When energetic, charged particles 
traverse the LAr medium, ionization electrons are produced and move
along the external electric field towards the anode planes. (right) The ionization
electrons pass through the induction wire planes and are  collected by the 
final collection wire plane. 
During this process, signals are measured on the wires
in each plane which provides information about the 3D positions and
energies of initial particles.}
\includegraphics[width=0.48\textwidth]{TPC_1.png}
\includegraphics[width=0.48\textwidth]{TPC_2.png}
\end{cdrfigure}


Figure~\ref{fig:signal_formation} illustrates the major elements of the processes 
involved in forming the TPC signals. When the ionization electrons drift through the 
wire planes, current is induced on the nearby wires. This process is described by the 
field response functions. The physics of the current induction is described by the 
Shockley-Ramo theorem~\cite{Shockley,Ramo}.  For an element of ionization charge, 
the instantaneous, induced current $i$ is proportional to the amount of that
charge $q$: 
\begin{equation}
i = q \cdot \vec{E}_{w} \cdot \vec{v}_q.
\end{equation}
The proportionality factor is product of the weighting field vector $\vec{E}_{w}$ 
at the location of the charge and its drift velocity vector $\vec{v}_q$. 
The weighting field vector $\vec{E}_{w}$, which depends on the geometry of the electrodes, 
can be calculated by removing the charge,  placing the potential of the targeted 
electrode to the unity potential, and setting all other conductors to ground. 
Figure~\ref{fig:signal_formation} shows a calculated weighting potential $V_{w}$ that 
is linked to weighting field $\vec{E}_{w}$ as $\frac{dV_{w}}{d\vec{r}} = \vec{E}_{w}$ for one 
induction plane wire using a 2D simulation based on Garfield~\cite{garfield}. 
In this calculation, the wire pitch is assumed to be 3~mm. There are three wire planes 
with the first two being induction and the last one being collection plane.  

The induced current on the wire is received, amplified, and shaped by
a pre-amplifier. This part is described by the electronics response
function (see Figure~\ref{fig:ele_res}).  
The resulting signal waveform is then digitally sampled at
regular intervals.  This data is referred to as the raw digits.  The
goal of the charge extraction process is to recover the number of
ionization electrons that must have arrived at each anode plane at a
given sample time in order to produce the measured raw digits.  The
information regarding the number, location (in the directions transverse
to and in the plane of the wires) and sample time of ionization
electrons are then used as input to the event reconstruction chain.

\begin{cdrfigure}[The process of TPC signal formation.]{signal_formation}{The process of TPC signal formation (left). The panel on the 
right shows a cross sectional view of the three wire planes (red dots) along with the electric field (orange lines) and the weighting potential 
(green lines) for a single induction wire of the first induction wire plane.}
\includegraphics[width=0.8\textwidth]{Signal_Extraction.png}
\end{cdrfigure}
%\fixme{Left panel of figure should have difference in terminology shown in top most and bottom most box, e.g. "true no. of ionized elec" and "reconstructed ..." -TK }

\begin{cdrfigure}[Simulated electronics response function in the time 
domain at 4.7 mV/fC gain]{ele_res}{The simulated electronics response function in the time 
domain at 4.7 mV/fC gain. The front-end cold electronics are designed to be 
programmable with 4 different gain settings (4.7, 7.8, 14, and 25 mV/fC) and 
4 shaping time settings (0.5, 1, 2, and 3 us). The shaping time is defined as the time 
between peak and 5\% of the peak at the falling edge. For a fixed gain setting, 
the peak is always at the same height independent of the shaping time. }
\includegraphics[width=0.6\textwidth]{electronics_res.pdf}
\end{cdrfigure}


While the principle is straightforward, calculating the measured
current itself can be very complicated. As shown in
Figure~\ref{fig:signal_formation}, the weighting field becomes smaller
at locations further away from the wire of interest.  
The weighting field also extends beyond the ``boundary'' of the wire.
Wire boundaries are defined by imaginary planes parallel to a wire,
perpendicular to the wire's plane and halfway between two neighboring
wires; i.e.,  in an ideal case, all charge produced within a wire's boundary
will drift to its nearest associated wire. 
%Due to the extent of 
Since a weighting field extends beyond a given wire's boundary, electrons drifting inside
this boundary can induce current in other wires.  
The induced currents therefore strongly depend on the local ionization
charge distribution near the wire of interest, which in turn depends
on the event topology of the initial energetic, charged particles.
%This fact makes the induced currents strongly depend on the local ionization charge distribution near the wire of interest, 


To illustrate the complication of the induction plane signal,  
an ideal track with a uniform charge distribution along it %the track 
is shown as 
an example in Figure~\ref{fig:ideal_track_1}. In the left panel, the 
two black lines represent the boundaries of one wire's region. In this case,  
%if one just counts 
counting only the ionization charge distribution within the wire's boundaries,
the expected 
distribution is shown in panel a) at top right.  However, the induced current on the wire of 
interest depends on the weighting field, which is smaller when the ionization electron is 
further away from the wire itself. Therefore, the effective charge distribution seen by 
the wire after considering the strength of weighting potential 
 would be similar to what is shown in panel b) on the right side of 
Figure~\ref{fig:ideal_track_1}. 
%\fixme{Why is signal in b) symmetric, when weighting potential for shown track is not ? - TK}
However, the wire of interest will experience an 
additional induced current from ionization electrons 
drifting outside its boundaries and in the regions of nearby wires. 
Since these ionization electrons are further away, 
the weighting field is even smaller and thus the induction from them is 
also smaller. A realistic effective charge distribution will be similar to the one shown in panel c) on 
the bottom right side of Figure~\ref{fig:ideal_track_1}. 


When the bipolar induction field response function is taken into account the 
charge transients change shape.
In the left panel of Figure~\ref{fig:ideal_track_2}, the top half shows 
the real charge distribution going through the targeted wire region. The convolution of this 
distribution with a bipolar response function will lead to results shown at the bottom. In this 
case, it can be seen that the signal height is still large at least for the start and the end of the 
signal. In the right panel of Figure~\ref{fig:ideal_track_2}, the top half shows the more 
realistic effective charge distribution seen by the targeted wire. The convolution of this 
distribution with a bipolar response function will lead to results shown at the bottom. In 
this case, it is apparent that the signal height is much smaller though the length of the signal is 
longer. This effect leads to complications in designing the data compression algorithm.

\begin{cdrfigure}[Induction plane field response for an ideal track (1)]{ideal_track_1}{Illustration of the induction plane field response for an ideal track (red arrow).}
  \includegraphics[width=0.7\textwidth]{ideal_track.png}
\end{cdrfigure}

\begin{cdrfigure}[Induction plane field response for an ideal track (2)]{ideal_track_2}{Illustration of the induction plane field response for an ideal track.}
\includegraphics[width=0.75\textwidth]{ideal_track_2.png}
\end{cdrfigure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\input{tpc-signal-extraction.tex}

%   It is:    \section{TPC Charge Extraction}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%--- insert section on calibration strategy ---%%%%%
\input{calibration_strategy}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Space charge effects}

%%%%%%%%%%%%%%%%%%%%%%%%
%%%\subsection{Introduction} 
\label{sec:SCEintro}

In order to correctly reconstruct the trajectories of particles that travel through the active volume of the TPC as well as precisely determine calorimetric information for these particles, it is essential to know very well the magnitude and direction of the drift electric field throughout the TPC bulk.  Nominally the electric field should be uniform throughout the TPC volume.  However, field effects such as the space charge effect (SCE) may cause distortions in the electric field that result in distortions in the reconstructed position of ionization electron clusters detected by the TPC wire planes as well as variation in the relative level of electron-ion recombination in different parts of the TPC~\cite{KirkSCE}.  The space charge effect is the build-up of slow-moving positive ions in a detector due to, for instance, ionization from cosmic muons.  As ProtoDUNE-SP is a detector on the surface with little overburden, the cosmic muon flux is expected to create a significant amount of space charge (positive argon ions) that could modestly impact the drift electric field within the TPC active volume.

In principle this effect could have modest impact in any TPC (liquid or gaseous) if the dimensions of the detector -- in particular the maximal drift distance -- are large enough to accumulate a high ion density.  In these cases, having a robust calibration method is necessary in order to account for the effect in particle trajectory reconstruction and calorimetry.  An example of the impact of the space charge effect on track reconstruction is shown in Figure~\ref{fig:SCEtrackEffects}~\cite{Mooney:2015kke}.  It should be understood that observations of these spatial distortions in data may include other effects, e.g., distortions of the applied field due to geometric and electric potential errors, distortion of the wire geometry, etc.  Within the context of this section, these other possible sources of distortions in reconstructed ionization electron cluster position are ignored as they are expected to be small in comparison with the distortions caused by the SCE.

\begin{cdrfigure}[Impact of the space charge effect on reconstructed tracks in the detector.]{SCEtrackEffects}{Impact of the space charge effect on reconstructed tracks in the detector.  The impact on a reconstructed track can be broken up into two distinct features:  a squeezing of the sides of the tracks in the transverse TPC directions that can somewhat resemble a rotation (``A'') and a bowing of the track toward the cathode that is most pronounced in the middle of the TPC (``B'').}
\includegraphics[width=0.99\linewidth]{trackSCE.pdf}
\end{cdrfigure}


%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Simulation} \label{sec:SCEsim}

Software was developed~\cite{SCEsimNote} to simulate the impact of space charge on the electric field within the TPC, along with the distortions in reconstructed ionization electron position at different points within the TPC bulk.  This simulation makes use of a Fourier series solution to the boundary value problem to solve for the electric field on a three-dimensional grid within the bulk of the TPC, an interpolation in between the grid points using radial basis functions to find the electric field everywhere in the TPC, and ray-tracing using the RKF45\footnote{``RungeKuttaFehlberg 4(5)'' method, an algorithm for the numerical solution of ordinary differential equations.} method in order to simulate the distortions in reconstructed position of ionization electron clusters.

An assumption is made that the charge deposition rate from cosmic muons is uniform across the TPC volume:  $2{\times}10^{-10}~\mathrm{C}/\mathrm{m}^{3}/\mathrm{s}$ at a drift field of 500~V/cm~\cite{KirkSCE}.  As a result, ignoring higher-order effects of the electric field distortions on the space charge configuration itself, the space charge density is linear with respect to the distance from the anode plane.  The space charge density profile used in the simulation is shown in Figure~\ref{fig:simSCDist} for a drift field of 500~V/cm.

\begin{cdrfigure}[Space charge density $\rho$ as a function of the $x$ position assumed in the simulation]{simSCDist}{Space charge density $\rho$ as a function of the $x$ position assumed in the simulation. The space charge density at the cathode, $90$ $\mathrm{nC}/\mathrm{m}^3$, reflects both the expected rate of cosmic ray charge deposition and effects of recombination~\cite{KirkSCE}. The distribution is independent of $y$ and $z$ in the simulation (an approximation).}
\includegraphics[width=.6\textwidth]{SCprofile.png}
\end{cdrfigure}


Some of the simulation results are shown in Figure~\ref{fig:simexample_Evals} and Figure~\ref{fig:simexample_Dvals}, which illustrate the impact of space charge on both the drift electric field (Figure~\ref{fig:simexample_Evals}) as well as the distortions in reconstructed ionization electron cluster position (Figure~\ref{fig:simexample_Dvals}).  At a drift field of 500~V/cm (corresponding to expected conditions during data-taking at protoDUNE), the expected maximal impact on the electric field is roughly 10\% in both the drift and transverse directions.

\begin{cdrfigure}[Simulated effects of space charge on the drift electric field in the ProtoDUNE-SP TPC]{simexample_Evals}{Illustration of the simulated effects of space charge on the drift electric field in the ProtoDUNE-SP TPC.  Results are shown for the effect in $x$ (top row), $y$ (middle row), and $z$ (bottom row).  The electric field distortions are normalized to the nominal drift electric field magnitude ($E_{0}$) of 500~V/cm and are plotted as a function of the true position in the TPC.  Simulation results are shown both for a central slice in $z$ (left column) and for a slice in $z$ closer to the end of the TPC, $z$ = 19 cm (right column).}
\includegraphics[width=.41\textwidth]{Ex_center_ProtoDUNE_E500.pdf}
\includegraphics[width=.41\textwidth]{Ex_end_ProtoDUNE_E500.pdf}
\\
\includegraphics[width=.41\textwidth]{Ey_center_ProtoDUNE_E500.pdf}
\includegraphics[width=.41\textwidth]{Ey_end_ProtoDUNE_E500.pdf}
\\
\includegraphics[width=.41\textwidth]{Ez_center_ProtoDUNE_E500.pdf}
\includegraphics[width=.41\textwidth]{Ez_end_ProtoDUNE_E500.pdf}
\end{cdrfigure}

\begin{cdrfigure}[Simulated effects of space charge on distortions in recon ionization e- cluster position]{simexample_Dvals}{Illustration of the simulated effects of space charge on the distortions in reconstructed ionization electron cluster position in the ProtoDUNE-SP TPC.  Results are shown for the effect in $x$ (top row), $y$ (middle row), and $z$ (bottom row).  The distortions in reconstructed ionization electron cluster position are shown in units of cm and are plotted as a function of the true position in the TPC.  Simulation results are shown both for a central slice in $z$ (left column) and for a slice in $z$ closer to the end of the TPC, $z$ = 19 cm (right column).}
\includegraphics[width=.41\textwidth]{Dx_center_ProtoDUNE_E500.pdf}
\includegraphics[width=.41\textwidth]{Dx_end_ProtoDUNE_E500.pdf}
\\
\includegraphics[width=.41\textwidth]{Dy_center_ProtoDUNE_E500.pdf}
\includegraphics[width=.41\textwidth]{Dy_end_ProtoDUNE_E500.pdf}
\\
\includegraphics[width=.41\textwidth]{Dz_center_ProtoDUNE_E500.pdf}
\includegraphics[width=.42\textwidth]{Dz_end_ProtoDUNE_E500.pdf}
\end{cdrfigure}



While the simulation provides a useful order-of-magnitude estimation of the distortions in electric field and reconstructed ionization electron cluster position within the ProtoDUNE-SP TPC, and provides basic shape features that we might expect in the data, there are several understood limitations of the simulation.  First of all, the flow of liquid argon, which may move positive argon ions in or out of the active TPC volume, is not considered.  Also, the assumption of uniform charge deposition from cosmics throughout the TPC may not be the case in reality, as enhanced cosmogenic activity near the top of the detector may lead to greater ion production rates closer to the top of the TPC active volume.  Finally, the linear space charge density assumed in the simulation (see Figure~\ref{fig:simSCDist}) is not quite correct; this approximates the ion drift speed (roughly 8~mm/s at a drift field of 500~V/cm) as constant throughout the TPC, while in reality the electric field distortions arising from the SCE itself would break this assumption.  With that in mind, comparisons of the simulation to first data collected at MicroBooNE show good agreement in terms of both magnitude and shape, looking at the top and bottom of the MicroBooNE TPC, with minor discrepancies due to what is believed to be effects of liquid argon flow moving space charge outside of the TPC active volume~\cite{SCEnoteMicroBooNE}.

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Calibration} \label{sec:SCEcalib}
\fixme{ minimize reference to laser system}

In order to correct SCE distortions (both electric field and reconstructed ionization electron cluster position) in data, a robust calibration scheme is necessary.  With information about the true position of ionization within the TPC in hand, as well as the reconstructed position of the ionization, spatial distortions of ionization deposition position can be extracted throughout the TPC active volume.  These spatial distortions can then be used to calculate the amount of electric field distortion throughout the TPC active volume.  Together, these two distortion maps can be used to correct track angles and calibrate out the variation in recombination and scintillation light yield throughout the TPC.

The strategy outlined above necessitates knowing both true and reconstructed ionization electron cluster positions throughout the TPC active volume.  This information can be obtained by using either cosmic muons or laser tracks.  In the case of cosmic muons, the ends of the tracks at the edges of the TPC active volume can be used to determine the spatial offsets due to SCE in the parts of the TPC where the transverse SCE is expected to be largest (see Figure~\ref{fig:simexample_Dvals}).  This first requires determining the $t_0$ of the cosmic muon, which can be obtained by either using a light-collection system or an external tagger (such as scintillator paddles located outside of the cryostat).  In the case of laser tracks, the true laser path through the TPC is known, allowing for calibration of spatial offsets due to SCE in the bulk of the TPC.  Together, cosmic muons and laser tracks (from e.g., a UV laser system installed at opposite ends of the cryostat~\cite{Ereditato:2014lra}) can be utilized to obtain SCE corrections throughout the entire TPC active volume.

Such calibration techniques discussed above require that the disortions due to SCE be relatively stable over time.  Preliminary observations at MicroBooNE suggest that this is the case on the timescale of several months~\cite{SCEnoteMicroBooNE}, though for a different cryogenic system.  This last point is important to note as the liquid argon flow pattern may be significantly different at ProtoDUNE-SP, leading to a space charge profile that may be time-dependent.

%%\subsection{PDS Light Extraction}

%%%% insert detector parameter calibration studies/measurements %%%
\input{detector_calib}



==> detector_calib.tex <==

\section{Detector-physics studies and calibrations}

Electromagnetic showers are relatively well-understood and can be used to understand the detector response.

	\subsection{ADC to energy calibration}
		\paragraph{Stopping/decaying muons}
		\paragraph{Michel electrons}

Neutrinos produced in supernova burst (SNB) explosions are calculated to be in the few-to-30-MeV range.
The DUNE Far Detector is expected to have a unique sensitivity to the $\nu_e$'s from an SNB in our galaxy.
%
The test beam cannot offer a sample of such low-energy electrons, but Michel electrons produced by decaying stopped muons are ideal for calibrating electron response in the appropriate 10-50~MeV energy range. 
The required  sample of low-energy muons will supply the 1400 Michel electrons needed for a 1\%  calibration of electrons in this energy range. This sample can be compared to a similar Michel electron sample
stemming from stopping cosmic muons.


	\subsection{Detector response uniformity}
		\paragraph{E-field response/space charge effects}
		
		A robust procedure to validate the TPC field response function is required be developed: \\
Field response on the induction plane is very complicated but holds the key to achieving a robust TPC  signal processing and thus the overall event reconstruction. It is, therefore, important to develop a 
program to calculate, calibrate, and validate field response functions. This validation of the field response function can be achieved by comparing the measured average response functions for cosmic muons with the simulated
ones. 

%%% \item [Measure field distortion effect (space-charge, LAr flow, beam window effect, etc).] 

The protoDUNE-SP detector will be placed on surface and effects coming from the space-charge modification of the electric field, or the effect of the choice of the location and design of the beam window will need to be included. The effects and strategies how to approach them are described in sections 3.5 and 7.1.
		
		\paragraph{APA alignments}

	\subsection{LAr purity monitoring}

	\subsection{Diffusion studies}

	\subsection{Noise studies}
  
  The ENC generated beyond the cold preamplifier is required to negligible ($<$ 50\%~\footnote{Since the noise from each source are added in quadrature, an extra electronic noise with less than 50\% of intrinsic cold preamplifier
noise would lead to less than 10\% increase of the total noise.}) compared to the 
expected ENC generated from the cold preamplifier in $>$ 95\% of the channels: \\
The only irreducible electronics noise is coming from the preamplifier on the TPC wires. It is thus
crucial to optimize the overall system to reduce the noises generating from other sub-systems. 
Lariat achieved such a performance with about a total of 500 channels. 

\fixme{xxxxxx Is any of the following text useful ??? xxxxxxxxx}
All the past or current large LArTPC experiments (ICARUS, MicroBooNE, and DUNE-35ton) have suffered from a sizable
number of unusable channels ($>$ 10\%) for %due to various reasons such as high noise, dead electronics, and disconnected wires. At the same time, each of the experiment achieved successes in reductions of the problems that cause some of the wires to be unusable. 
For example, ICARUS has no disconnected wires. In LAriat, all cold electronics channels ($\sim$ 500) are live and achieve the expected $\sim$400 electrons equivalent noise charge (ENC). In the ATLAS LAr calorimeter, only about 0.1\% of the cold electronics channels are unusable. 
In MicroBooNE, the ENC after software noise filtering is about 400 electrons, which is consistent with the design specification of the cold electronics. Also, all the major sources of electronic noise
have been identified, and hardware solutions are in order. Therefore, with careful and systematic quality assurance and controls, it is possible to reduce the total number of unusable channels
by at least one order of magnitude. This is one of the primary goals of ProtoDUNE.

\fixme{the above is not clear. 
It needs a progression something like this:
`All these detectors have had channel problems. Problems have been identified and are fixed. From this we know we can reduce unusable channels by order of magnitude.' The sentence about successes is confusing: success after fixing? Or success in other areas? DONE(?)
}



	\subsection{Recombination}
	 (angular dependency)




==> execsum.tex <==
%\chapter{execsum}
This is the executive summary.  Write me.


==> organization.tex <==
%\chapter{organization}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{ProtoDUNE-SP organization}

Given its technical challenges, its importance to the DUNE experiment and the timeframe in which it must operate, protoDUNE-SP requires a strong organizational structure with effective leadership to ensure its success. This detector is similar in design to the Short Baseline Neutrino Detector (SBND), the near detector of the SBN experiment at Fermilab. 
\fixme{It may b better to reword this in a less FNAL centric way and emphasize the similarity with the dual phase first, then mention the 
fertile ground that the neutrino platform provides and in that context mention SBND as well.}
The timelines of the two experiments are very similar, and therefore the development of effective synergies, in particular, the exploitation of common detector solutions, common test tooling, and the optimal use of resources (human and financial) will help to achieve the goals of both efforts.  The full description of the protoDUNE-SP organization is in~\cite{pdune-sp-org}.

%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{A Detector Organization within the DUNE Collaboration}

ProtoDUNE-SP is a detector organization within the DUNE collaboration, at the same level as the Far Detector (FD), Near Detector (ND) and ProtoDUNE-DP organizations, as indicated in Figure~\ref{fig:hi-lev-org-det}. The ProtoDUNE-SP effort is led by three Coordinators, supported by a Deputy, and by a Technical Lead.

\begin{cdrfigure}[High-level organization of the detector efforts within DUNE]{hi-lev-org-det}{High-level organization of the detector efforts within DUNE. Each has a structure of working groups (WG) beneath, dedicated to particular subsystems or components.}
 \includegraphics[width=0.95\textwidth]{hi-lev-org-det}
\end{cdrfigure}
%%\fixme{In fig 8.1: DUNE FD coordinator singular?; also I thought we were standardizing on ProtoDUNE not protoDUNE. Anne}

The main ProtoDUNE-SP detector elements (TPC, CE and PDS) are intended as engineering prototypes for the DUNE FD. The DUNE FD organization is responsible for the management of the production of these detector components. The ProtoDUNE-SP organization is responsible for the activities at CERN, including the detector integration, installation, commissioning and operation of the experiment in the charged-particle test beam at the Neutrino Platform.  This also includes interfaces to DUNE Physics and DUNE Computing \& Software organizations. Efficient coordination between the ProtoDUNE-SP and FD organizations is key to success of this project.



Each member of the ProtoDUNE-SP leadership has a distinct role:
\begin{itemize}
\item The DUNE Technical Board (TB), chaired by the DUNE Technical Coordinator, will act as the main decision-making body for the design of the ProtoDUNE-SP detector. All major decisions regarding the design of ProtoDUNE-SP will take place in the TB, which is responsible for the careful evaluation of all technical aspects and prompt selection of available alternatives during the design and construction phases. Both the DUNE FD and the ProtoDUNE-SP leadership are members of the TB, ensuring that all stakeholders are involved in the decision-making process.
\item The ProtoDUNE-SP Coordinators effectively act as spokespersons for the ProtoDUNE-SP project and report to the DUNE management. They are ex-officio members of the DUNE Technical Board (TB).
\item The ProtoDUNE-SP Deputy Coordinator supports the ProtoDUNE-SP coordinators as required and, in addition, oversees the ProtoDUNE-SP scientific activities. 
\item The ProtoDUNE-SP Project Manager is responsible for all project management aspects for ProtoDUNE-SP. He or she maintains and is responsible for the overall schedule for ProtoDUNESP; represents ProtoDUNE-SP in the Far Detector international project management; manages the ProtoDUNE-SP work at CERN and liaises with the CERN teams responsible for the Neutrino Platform infrastructure for installation and operation of ProtoDUNE-SP.
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Synergies with ProtoDUNE-DP}

Concurrently with ProtoDUNE-SP, ProtoDUNE-DP will address a complementary part of the DUNE strategy for reaching the design goal of a 40-kt fiducial mass detector. ProtoDUNE-SP and ProtoDUNE-DP share space in the EHN1 experimental hall.  The CERN Neutrino Platform offers great opportunities for utilizing common infrastructures (e.g., the cryogenics system, LAr purification, DAQ, computing) and for an optimal use and sharing of engineering and scientific resources during assembly, commissioning and operation.

As mentioned, ProtoDUNE-SP and ProtoDUNE-DP are placed at the same high level as the far and near detector organizations in the DUNE organizational chart. This fosters a strong coupling and overlap between the two ProtoDUNEs as well as between them and the Far Detector working groups and their activities. It should be noted, however, that the ProtoDUNEs (SP and DP) are identified as distinct organizations that take ownership of and responsibility for their separate experiments.

During a meeting of the two ProtoDUNE management teams at CERN in February 2016, it was agreed that the organizations would pursue common development in several areas either through new joint working groups of the DUNE collaboration or existing working groups, as follows.


\begin{itemize}
\item Online Computing \& Disk Storage -- Joint Working Group
\item Offline Computing -- Common development through DUNE Software \& Computing Working Group
\item Slow Controls -- Joint Working Group
\item DAQ -- Independent efforts but potential for using common software tools
\item High Voltage Delivery -- Joint Working Group
\item Beam Configuration and Instrumentation -- Joint Working Group
\item Field Cage -- Common development through Far Detector CPA/FC/ HV Working Group
\item Beam Window and Plug -- Common development for ProtoDUNEs through Far Detector
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Integration with CERN's Neutrino Platform}

As the ProtoDUNE-SP Project Manager is responsible for all project management aspects for ProtoDUNE-SP, he or she is the primary liaison with the CERN teams responsible for the Neutrino Platform infrastructure for installation and operation of ProtoDUNE-SP. \fixme{expect updates here}

%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{ProtoDUNE-SP Teams and Leadership Responsibilities}

The ProtoDUNE-SP work is divided into several major tasks, each of which has a dedicated team, as illustrated in Figure~\ref{fig:pDUNE-SP-org}.

\begin{cdrfigure}[ProtoDUNE-SP Organization Structure]{pDUNE-SP-org}{ProtoDUNE-SP Organization Structure}
  \includegraphics[width=0.95\textwidth]{pDUNE-SP-org.jpeg}
\end{cdrfigure}

\fixme{Find new org chart per Jolie}

%%%%%%%%%%%%
\paragraph{Detector Integration, Testing and Installation (DITI)}

This CERN-based Detector Integration, Testing and Installation (DITI) team is led by a coordinator, with assistance from the installation team leader, other coordinators and Detector Team Leaders.  This team will lead DAQ, installation and engineering integration activities starting from the arrival of the detector components at CERN through to the detector commissioning.

The Technical Lead provides the interface to CERN in all matters related to the infrastructures in the assembly hall and in the experimental hall at the Neutrino Platform, including the cryostat and the cryogenics and LAr purification systems.

Specific team members based at CERN provide the interface between the DITI team and each of the DUNE Far Detector WGs responsible for delivering the ProtoDUNE-SP detector components. 

Correspondingly, the TPC, Photon Detection System and cold electronics WG leaders for the DUNE FD are ex-officio members of the ProtoDUNE-SP DITI managerial structure, ensuring a direct connection. The DITI team includes members (based at CERN) who take responsibility for the major detector components once they are at CERN.

Team leaders for other detector components lead integration, testing and installation work for APA, HV/FC/CPA, photon detector, photon electronics and Cold Electronics.


%%%%%%%%%%%%
\paragraph{High Voltage, Cryogenics, Beam Window and DAQ }

The high voltage (HV) System, Cryogenics System, Beam Window and DAQ are managed by dedicated ProtoDUNE-SP teams. Where appropriate, these teams may overlap with the corresponding ProtoDUNE-DP teams. Team leaders take the responsibility for the timely and technical success of their task. The team leaders will be invited to the DUNE Technical Board meetings when matters relating to ProtoDUNE-SP are discussed.

%%%%%%%%%%%%
\paragraph{Other Tasks}

\begin{itemize}
\item If a Cosmic Muon Tracker/Trigger is implemented for ProtoDUNE-SP, a separate team will be set up mirroring those for the HV and other systems. \fixme{need to clearly state that there will be a muon tagger or scratch this item - NOTE: muon tagger hardware described in section 4}

\item Dedicated ProtoDUNE-SP teams have been set up for the Computing Infrastructure and for Beamline Detectors. They will provide the interface with CERN IT and with the Neutrino Platform and will support the experiment during run operations.
\item The ProtoDUNE-SP physics planning and analysis will be led by Software Development and Physics teams. They will take responsibility for the preparations and fast delivery of detector performance characterization and physics results based on beam and cosmic ray data.
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Cost estimate}

%%%%%%%%%%%%
\paragraph{ProtoDUNE-SP costs by subsystem}

The Memorandum of Understanding (MOU) for Collaboration in the Neutrino Program, signed by Sergio Bertolucci and Nigel Lockyer in December 2015 outlined ProtoDUNE-SP CORE costs by subsystem and funding agency.  The CERN Neutrino Platform is providing significant deliverables to enable the successful execution of the DUNE prototyping program, including the experimental hall, beamline, cryostat support structure, and membrane cryostat.  In addition, CERN is providing a significant portion of the cryogenics plant, the cathode plane assemblies, field cage tooling, feedthroughs, DAQ, installation resources, online data processing support, and detector slow controls.  

The costliest element aside from the cryostat and cryogenics, the Anode Plane Assemblies, are being provided by the United States (US-DOE) and the United Kingdom.  The US-DOE is fully funding the Cold Electronics production.  The UK is leading the DAQ system effort, with contributions from the US.  The table shown in Figure~\ref{fig:mou}, from the referenced MOU, outlines the costs and contributing institutions.

\begin{cdrfigure}[Costs and contributing institutions]{mou}{Costs and contributing institutions \fixme{table is outdated as far as institutional responsibilities go - should be updated or a sentence added in text that it has been revised.}}
\includegraphics[width=0.8\textwidth]{MOU-picture}
\end{cdrfigure}

%%%%%%%%%%%%
\paragraph{ProtoDUNE-SP operations support}
To enable the success of protoDUNE-SP integration, installation and commissioning activities, the DUNE Collaboration and DUNE Project representatives have requested supplemental funding from the US Department of Energy to support scientist travel to CERN and consumables for the protoDUNE-SP run.  This funding is also intended to support extended scientific personnel stays at CERN for personnel that are not supported by the DUNE project or university research grants. 

In addition, the operations funding request included allocations for consumables such as liquid argon and liquid nitrogen, as well as computing equipment and supplies.  The request is under consideration by US DOE.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{ProtoDUNE and EHN1 schedule}
\subsection{Schedule}

The schedule summary in Figure~\ref{fig:schedule} outlines the timeline for high-level activities at CERN for ProtoDUNE-SP, including test stands, integration activities, installation and commissioning.  The Detector Integration, Testing and Installation Coordinator, with the system team leaders and the ProtoDUNE-SP Coordinators, is developing a detailed testing protocol and sequencing plan for components.  Detector components will start arriving at CERN in early 2017, and the clean room set up and component testing will start in March 2017. The beam data-taking operation is scheduled to run from the beginning of August 2018 through the end of October 2018.

\begin{cdrfigure}[Schedule summary]{schedule}{Summary of schedule for high-level activities at CERN for ProtoDUNE-SP}
\includegraphics[width=0.95\textwidth]{protodune-sp-schedule-for-tdr}
\end{cdrfigure}

==> quality.tex <==
The quality control and quality assurance procedures for the individual components of the ProtoDUNE-SP detector are collected in this chapter.

%%%%%%%%%%%%%%%%%%%%%%%%
\section{APA}

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{General}

Each ProtoDUNE-SP APA will be subject to a testing program during production that will demonstrate their compliance with the design and manufacturing requirements for the experiment.  Given the large size of the APAs, and the highly specialized cryogenic and electronic infrastructure necessary for their designed operation, the testing plan followed during production is necessarily targeted at those features of the APAs which can be addressed prior to final installation in the cryostat.  A separate suite of testing, in a cryogenic environment, is planned to be conducted at CERN, as described in ???? \fixme{is there a section in the TDR for this cold-box test?}.

The tests described in this section will be conducted on APAs during construction, as well as on completed APAs.  Subcomponents ($e.g.$ - wire boards, BeCu wire, etc..) are verified or tested by the appropriate vendor or subsystem manager prior to their use in APA construction.  Each APA will be subject to the testing listed in Table \ref{tab:apatesting}.   Many of the tests (e.g. - tension, continuity, isolation, position survey, bias voltage) are repeated as each successive wire layer of the APA is added, testing the newly installed wires as well as spot-checking wires from previously installed layers. The summary of the tests on each APA, and the associated data collecting during the tests, are recorded in a traveler.

\begin{cdrtable}[APA Testing]{llr}{apatesting}{Tests to be conducted on APAs during production.}
Label & Requirement & Test Method  \\ \toprowrule
Tension      & All wires must be tensioned to 5$\pm$1 N & Laser Survey \\ \colhline
Cryo       &  All APA must operate at 87 K  & Cryotest \\ \colhline
Electrical       & All wires electrically connected at top/bottom of APA  & Continuity \\ \colhline
Isolation & Neighboring APA wires have $\geq$1 M$\Omega$ resistance & Multimeter\\ \colhline
Voltage & Anode planes must hold $\geq$100$\%$ bias & Bias \\ \colhline
Position & All wires must be within 500 $\mu$m of design location & Survey\\ \colhline
Frame & APA frame satisfies all bow/twist/fold criteria & Survey\\ \colhline
\end{cdrtable}

 %%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Tests and surveys}

\fixme{Moved from chap 2}

 %%%%%%%%%%%%
 \subsubsection{Tension survey}

Wire tension is a critical parameter in the performance of the APA, and needs to be strictly controlled to ensure the detector will be robust to operation in a cryogenic environment.  As each wireplane layer is added to the APA, and before the next layer is added and restricts access, the tension of every newly added wire will be measured.  Any wire that is more than 1.0 N out of tolerance from the design value of 5.0 N will be removed and, if possible, replaced.  The tension measurement is performed using a laser-photodiode system, developed at PSL and integrated into the wire-winding apparatus, which will record the resonant frequency of a plucked wire.  Visible checks will also be made during production to identify any noticeably sagging wires.  Spot checks of tension will also be made after cryogenic testing at the production site, as well as at CERN prior to insertion of an APA into the ProtoDUNE-SP cryostat.  

 %%%%%%%%%%%%
\subsubsection{Electrical continuity test}

The electrical connection of each APA wire to the cold readout electronics must be verified to ensure a minimum ($<$0.5$\%$) of un-reachable channels in the completed detector.  Un-reachable wires (e.g. originating from cold solder joints or wires that are broken but held in place by epoxy bead) are distinct from clearly broken wires (e.g. obvious strands of wires hanging loose from the APA) which will be removed/replaced during production.   In addition to providing a pathway to record detector signals, wires receive their bias voltage via their connection to the readout electronics, which shapes the electric field in the anode region.  As such, disconnected wires impact the signals that surrounding channels will collect.  As each wireplane layer is added to the APA, and before the next layer is added and restricts access, the electrical connection of every newly added wire to the corresponding wire-bonding board will be verified.  Using a multimeter, or other equivalent methods, the continuity will be verified by directly probing between the ``bottom" end (i.e. - the end that terminates on the non electronics-plate end of the APA) of the wire and the signal trace on the wire-bonding board at the ``top" end (i.e. - the end that terminates on the electronic-plate end of the APA).  Any wire that fails this continuity test, by producing a resistance $>$ 500 $\Omega$ (using 4.4 $\Omega$/m resistance for BeCu wire that is 7.5 m long, and allowing margin for additional parasitic resistance), will be removed and, if possible, replaced.  Spot checks of continuity will also be made after cryogenic testing at the production site, as well as at CERN prior to insertion of an APA into the ProtoDUNE-SP cryostat.

 %%%%%%%%%%%%
\subsubsection{Electrical isolation test}

Each wire of the APA should be electrically isolated from every other wire, in order to avoid shorting out channels and potentially damaging the readout electronics.  Shorted-out wires will also impact the electric-field uniformity in the anode region, and can impact signals in surrounding channels.  Using a multimeter, or other equivalent methods, the isolation between each APA wire and adjacent wires will be measured and verified to have resistance $>$ 1 M$\Omega$.  Since a given wire has many adjacent wires, a dedicated circuit designed to expedite this test will be desirable.  Any wire failing this test will be removed and, if possible, replaced.  Visible checks will also be made during production to identify any touching wires.  Spot checks of isolation will also be made after cryogenic testing at the production site, as well as at CERN prior to insertion of an APA into the ProtoDUNE-SP cryostat.

 %%%%%%%%%%%%
\subsubsection{Wire position survey}

Knowledge of the position of every wire in the APA is required in order for physics analysis of data to be successful.  This information is utilized to create a description of the detector geometry inside the simulation software, and is the basis on which reconstruction algorithms are built. The preliminary description of the geometry assumes a perfect detector built according to the APA design drawings.  Any deviations from this design in the final as-built APAs needs to be incorporated into the software geometry.  All wires should be surveyed during production to verify they are within 500 $\mu$m of the design location.  This survey is partially accomplished by verifying the APA flame flatness is within specifications, and that the wire-bonding boards and support combs are located upon the frame in the desired position.  The APA will be surveyed using a Cognex camera integrated into the winding machine.  The camera employs machine vision to identify each pin/tooth on the installed wire-bonding boards, and from this data a map of wire location will be generated.  This survey should be performed as each wireplane layer is added to the APA, and before the next layer is added and restricts access.  Any wire that is more than 500 $\mu$m from the nominal location, according to survey data, should be inspected and if found to have problems, removed and replaced.  Visual checks throughout the wire-winding process will also be performed to identify any wires that appear out of place.

 %%%%%%%%%%%%
\subsubsection{Bias voltage test}

All wires on the APA must be able to reach their design bias voltage in order to achieve the desired electric-field uniformity and transparency conditions required for successful LArTPC operation.  Inability to reach the desired voltage could be an indication of component failure on the CR boards, or of wires in the APA being shorted out.  The CR boards should be tested prior to their installation on the APA to verify they can be biased to 100$\%$ of the largest operating voltage of any anode layer (e.g. the Collection layer's 820 V).  The components selected for the CR boards are chosen with margin about this operating point, to allow for bias voltages in the as-built detector to be adjusted, either for signal-shaping studies or for systematic studies of detector performance at various drift-field values.  As each wireplane layer is added to the APA, and before the next layer is added and restricts access, each newly added wire-bonding board should be connected to a CR board and biased to 100$\%$ of the largest operating voltage of any anode layer.  Any unexpected current draws observed will be traced to the originating wire(s), and if necessary, the offending wire(s) will be replaced.  Visual checks should also be performed during this test to verify that wires being biased do not deflect or move in any unexpected manner.  This test may be augmented when multiple wireplane layers are available, to verify that wires in adjacent layers do not develop unexpected cross-talk when biased.

 %%%%%%%%%%%%
\subsubsection{Cryogenic test}

The completed APAs must be robust to operation in a cryogenic environment.  Wires must be able to withstand the cooldown to liquid argon temperatures.  In order to verify the workmanship of each APA, a cryogenic test will be performed as each APA is completed and before shipment to CERN.  The APAs will be placed in a custom-built cold box, where they will be gradually cooled (at a rate consistent with requirements on keeping wire tension increases below a safe level) to $\sim$100 K (exact value to be determined).  The default plan is to use cold gas from a LN supply for this test, and flush gas through the cold box until it reaches the desired temperature.  The APA will be arranged in a horizontal orientation, as this simplifies the engineering of the cold box.  It is not anticipated that loading on the APA/wires due to gravity (e.g. from horizontal vs. vertical orientation) will lead to any significant changes in wire tension, and the frame will be supported appropriately.  The APA will be inspected after this cold test to verify that no wires have broken.  Spot-check tests of tension/continuity/isolation/bias will be performed to verify if any channels have changed relative to their pre cold-test values.  Criteria for acceptance after this test (e.g. number of problematic wires identified by this test) are under development.

 %%%%%%%%%%%%
\subsubsection{Testing at CERN}

Upon arrival at CERN, and prior to integration with interfacing subsystems (e.g. - light collection and electronics), each APA will be subjected to visual inspection, and spot-check ($\sim$10$\%$ of total channels) tests for wire tension, continuity, isolation, and bias voltage will be performed and compared to the equivalent pre-shipping values.




%%%%%%%%%%%%%%%%%%%%%%%%
\section{CPA}

The following activities are planned to assure the CPA meets all design requirements as defined in the fabrication drawings and description in the sections above:
\begin{itemize}
\item Performed 35 ton HV test at FNAL.
\item Fabricate four prototype CPAs to test the design and fabrication and assembly methods.
\item Installation test at Ash River:
\begin{itemize}
\item Test the lifting and handling of the four prototype CPA's.
\item  Load the 4 prototype CPA's with FC modules and test and evaluate their installation.
\end{itemize}
\item Develop a QC plan for inspecting every fabricated part of the CPA frame to make sure they meet the dimensions and tolerances on the fabrication drawings.
\item Develop a QC plan for inspecting and measuring each CPA module and completed CPA plane to ensure they meet the dimensions and tolerances on the drawings.
\item Perform tests of each joint in the CPA frame (see Section 3) to ensure that their design and strength meets the load requirements.
\item Create an integrated model of the entire TPC to evaluate interfaces and installation methods.  
\item Develop a QC for receiving the resistive panels.  Measure the dimensions to confirm they meet the drawings and setup a plan and acceptance criteria to insure that panel resistance is acceptable.
\item Develop a QC  HV test at CERN for evaluating side to side and top to bottom resistance for each completed CPA but after final assembly and after hanging during installation.  
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%
\section{FC}

The following activities are/will be performed to assure the field cage meets all design criteria as defined in the fabrication drawings and description in the sections above:
\begin{itemize}
\item	Fabricate prototype FCs to test the design and fabrication and assembly methods.
\item	Installation test at Ash River:
\begin{itemize}
\item	Test the lifting and handling of the prototype FCs.
\item	Mount the prototype FCs to the CPA modules and test and evaluate their installation.
\end{itemize}
\item	Develop a QC plan for inspecting every fabricated part of the FC frame to make sure they meet the dimensions and tolerances on the fabrication drawings.
\item	Develop a QC plan for inspecting and measuring each FC module and completed FC plane to insure they meet the dimensions and tolerances on the drawings.
\item	Perform tests of each joint in the FC frame (see Section XX) to insure that their design and strength meets the load requirements.
\item	Create an integrated model of the entire TPC to evaluate interfaces and installation methods.  
\end{itemize}

 %%%%%%%%%%%%%%%%%%%%%%%%%
\section{HV}

\fixme{no info contributed}

  %%%%%%%%%%%%%%%%%%%%%%%%%
\section{PDS}

\fixme{no info contributed}

%%%%%%%%%%%%%%%%%%%%%%%%%
\section{CE}

A full description of the testing procedures is being developed in a separate document. A 
summary is provided here.

%%%%%%%%%%%%%%%%%%%%%%%%%
\section{DAQ}

The DAQ for ProtoDUNE-SP does not require large numbers of custom hardware components to 
be built and tested.  There will be 8 COBs with 8 RCEs each, 2 FELIX cards, 24 SSPs, the timing 
and trigger systems and off-the-shelf hardware (computers, network switches, storage, etc.).
As such, a significant amount of automation is not needed to test and qualify the 
components.  

Qualification tests of the RCEs, FELIX boards, SSPs, timing and trigger systems will
be driven by the host institutes producing those systems.  Reception tests will be 
performed to identify any failures due to transport.  In order to fully qualify the 
boards, they will need to be individually tested with control samples.  Data generators
will be used in place of the front-end electronics where applicable.  Full data rate 
testing will be performed when the first full detector slice is in place at EHN1 (expected
Q2 2017).  Data challenges will take place during Q1 2017 in advance of the arrival of the 
first APA, and again as the computing system expands to its full capacity.

%%%%%%%%%%%%%%%%
\subsection{Prototype testing}
\label{subsubsec:ce_install_proto}

Dedicated test boards for the FE ASIC and ADC ASIC,
were used to characterize the performance of prototype ASICs at both 300~K and 77~K,
and taking them through multiple thermal cycles.
An automated test board was built for the FE ASIC (Fig.~\ref{fig:tpcce_FE_TestBoard})
to evaluate large numbers of FE ASICs at room temperature,
and another such board is currently being designed for the ADC ASIC (Fig.~\ref{fig:tpcce_ADC_TestBoard}).

\begin{cdrfigure}[FE ASIC testboard]{tpcce_FE_TestBoard}{FE ASIC testboard.}
\includegraphics[width=0.6\linewidth]{tpcce_FE_TestBoard}
\end{cdrfigure}
\begin{cdrfigure}[ADC ASIC testboard]{tpcce_ADC_TestBoard}{ADC ASIC testboard.}
\includegraphics[width=0.6\linewidth]{tpcce_ADC_TestBoard}
\end{cdrfigure}

The development of the FE and ADC ASICs has proceeded through a series of prototype designs.
A 128-channel prototype analog mother board has been developed and tested in the lab.
Together with an FPGA mezzanine in place of the digital ASIC mezzanine,
they form a FEMB for use in the protoDUNE TPC,
since the COLDATA work is unlikely to be advanced enough to
provide more than a fraction of the electronics needed for the aggressive protoDUNE schedule.
A test stand has been developed to test the FEMB
using a commercial FPGA evaluation board as a mini-DAQ system.
All evaluation test data are stored on a desktop PC and analyzed to
determine whether the board is ready to be installed on the detector.

During the prototype testing, a procedure has been developed for the production test of the cold electronics boards.
This includes key parameters (gain, noise, non-linearity, etc.) that should be tested,
detailed steps of the test to collect data and extract these parameters,
and also the work flows to perform the test at both 300~K and 77~K.

Prototype cold electronics has been tested with prototype TPC and DAQ system,
to evaluate the performance of the APA assembly, and help the development of the DAQ software.
A vertical slice test has been used as the test bed for the integration test.
It is an important step to identify potential issues, check out system integration and performance
before the installation into the cryostat.

%%%%%%%%%%%%%%%%
\subsection{CE assembly testing}
\label{subsubsec:ce_install_assembly}

The front-end readout boards will be thoroughly tested. A testing program has been identified:
\begin{itemize}
\item A small number of the ASICs will undergo a complete suite 
of tests, including thermal cycling to determine the batch yield.
\item If the yield is high ($>$ 95\%), all ASICs will be mounted 
on the front-end boards.
Tests will be performed on each board and bad chips replaced as needed.
\item If the yield is not high, an automated test fixture will be 
fabricated to validate every ASIC chip before mounting on the readout boards.
Board-level tests after mounting the ASICs will be conducted.
However, previous experience indicates that this scenario is very unlikely.
\item The fully assembled front-end boards will be thermally cycled multiple times while connected
to a simple DAQ system to ensure reliable operation.
\item After the front-end electronics boards have been installed on an APA,
an initial calibration of all electronic channels will be performed.
The electronic gains and noise levels of all channels will be recorded in a database.
\item Electronic calibration on all channels will be performed while the APA is cold and again after it is warmed up.
\end{itemize}

%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Beam plug}

As a part of the QC process for the beam plug, the vendor will conduct the following acceptance tests for the production units before shipping:
\begin{itemize}
\item {Initial helium leak check}
\item {Internal pressure check at cryogenic temperature (at about 2x operating pressure)}
\item {Post-test helium leak check to assess potential damage}
\item {External pressure check at room temperature (below 100 psi)}
\item {Final helium leak check to ensure no damage has been incurred}
\end{itemize}
The acceptable leak rate is below 15.6$\times 10^{-5}$ scc/s (He gas equivalent).
The tests performed by the vendor are primarily related to pressure safety and leak rates. Some of those tests will be repeated by LBNL upon receiving the units to verify vendor's results. In addition, LBNL will conduct tests to verify other aspects of the beam plug, in particular, the HV characteristics. The HV tests will be conducted using various facilities as described in the following sections.

\paragraph{BLANCHE Test Stand}
The BLANCHE test stand at Fermilab is a LAr cryostat dedicated to study high voltage related issues. It is 152 cm tall with a 76 cm inner diameter. The test stand is connected to a LAr purification system to remove oxygen and water contamination. The test stand is capable of delivering up to 150 kV to the sample. The cryostat is large enough to test a full size beam plug. The plan is to test the beam plug in BLANCHE to verify that the beam plug can withstand HV in LAr environment.
\\fixme{earlier nominal value across beam plug was said to be 165kV - so, test is not covering full range. Maybe add sentence to address this issue.}

\paragraph{Test in Charged Particle Beam}
During ProtoDUNE-SP physics runs, a charged particle beam will go through the beam plug with a rate of up to 100 Hz during a beam spill. The current induced from the ionization of the nitrogen gas by the charged beam particles is expected to be small; less than 1 nA during the spill. Given the low ionization rate and long pause between spills, we do not expect the charged particle beam to introduce electrical breakdown inside the beam plug. However, we plan to verify the design by putting the beam plug in a test beam with the beam plug at nominal HV. We will study the current flow inside the beam plug as a function of beam rate and nitrogen gas pressure. To minimize possible HV breakdown on the outer surface of the beam plug, which may complicate the interpretation of the test results, the beam plug will be immersed in dielectric oil. The test apparatus with the beam plug installed inside the setup is shown in Figure~\ref{fig:beamwindow_SLAC}.
\begin{cdrfigure}[SLAC beam test]{beamwindow_SLAC}{Beamplug test setup in electron beam to test electrical breakdown in the N filler gas.}
  \includegraphics[width=0.6\textwidth]{beamwindow_SLACtest}
\end{cdrfigure}

\paragraph{Full integration test in 35-ton cryostat}
The final QC test of the beam plug is conducted inside the 35-ton cryostat at Fermilab. A small field cage mock-up is constructed and assembled inside the cryostat along with the beam plug. For this test, the beam plug is mounted to the field cage using a mounting scheme which is identical to the ProtoDUNE-SP one. The field cage mock-up will only have the first 10 profiles of a TPC, however, they will be operating at the nominal voltages. Therefore, the planned test will be a full-field test with the beam plug integrated into the field cage and the rest of the HV systems. A successful test would entail operating the TPC at the nominal HV (CPA at -180 kV) with the beam plug attached and that the electrical performance of the field cage with and without the beam plug is functionally the same.

\begin{cdrfigure}[PC4 Test setup]{beamwindow_PC4}{Field cage mock-up high voltage test in 35-ton cryostat \fixme{preliminary drawing}.}
  \includegraphics[width=0.95\textwidth]{beamwindow_PC4Test}
\end{cdrfigure}

%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Cryogenics and LAr purification systems}

%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Scope}

The project follows the CERN QA/QC plan. Additionally, specific Neutrino Platform Cryogenics documentation control policies have been developed to ensure that the documentation is circulated and archived properly. A design plan is also being developed to ensure that the design is performed according to the specifications.\\
%
External companies will be contracted for the design, fabrication, delivery, installation and testing of the cryogenic system, one for the proximity and external cryogenics and one (could be the same) for the internal cryogenics.

The following sections are extracts from the \textit{Quality Assurance} section of the Invitation to Tender for the proximity and external cryogenics and the Price Enquiry for the internal cryogenics~\cite{invit-tender-cryo}.

%%%%%%%%%%%%%
\paragraph{General}

The contractor shall have or shall guarantee that its sub-contractors (when applicable) have a valid ISO 9001:2008 (or later) certifications issued by a recognized certification body in the scope of the supply for \"design, engineering, production, installation, sales of vacuum systems, cryogenic equipment and transfer lines\".

%%%%%%%%%%%%%
\paragraph{Scope}
A dedicated quality plan must be prepared by the contractor as per requirements.

%%%%%%%
\paragraph{Definition}
A quality plan describes the operational quality system to ensure that:
\begin{itemize}
\item Contract requirements will be met.
\item Evidence of such compliance is maintained.
\end{itemize}
It covers the whole scope of the contract.

%%%%%%%
\paragraph{Content of the quality plan}
\begin{itemize}
\item The specific allocation of resources, duties, responsibilities and authority.
\item Details of all sub-contractors and how interfaces will be managed if any.
\item The specific procedures, methods and work instructions to be applied.
\item The specific procedures for inspection and testing.
\item The specific methods of communication and testing
\item The design and performance margins.
\end{itemize}


%%%%%%%
\paragraph{Quality management}

The plan shall:
\begin{itemize}
\item Identify the key individuals responsible for ensuring the activities performed during the contract.
\item Show an organization flow chart to facilitate understanding.
\end{itemize}

%%%%%%%
\paragraph{Deviations and non-conformities}

The plan shall indicate how, when and by whom deviations and non-conformities will be processed including those originating from subcontractors, if any.

%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Cryo and LAr purification inspection and controls}

Specific control points apart from the ones required by the chosen applicable standards and Pressure Equipment Directive (PED) Essential Safety Requirements
 will be performed during the fabrication and installation phases. Every specific inspection or control will be covered by a dedicated procedure developed by the manufacturer and approved by CERN. In case of non-conformities (i.e., non-compliance with specified requirements), a corresponding non-conformity report will be issued by the manufacturer.

The contractor will ensure a close oversight of the manufacturing. This monitoring will include Notification Points (NP) and Hold Points (HP).

A NP is a milestone where the contractor is required to notify CERN that it has completed a specific task or a specific deliverable and is proceeding to the next task or to the next action on the specific deliverable. A NP is meant to enable CERN personnel to follow the progress of the contract and possibly to witness a critical manufacturing step at the contractor' s premises. A NP will not affect the production flow of the contractor that will continue the work even without a reply from CERN. 

A HP is a milestone where contractor is required to notify CERN that it has completed a specific task or a specific deliverable and must stop the associated processes until a HP Clearance is issued. The HP Clearance will be issued on the basis of clearly identified Quality Control, data and acceptance test results to be provided to CERN at the time of the request. In case of clearance, the contractor will resume its activity. In case of rejection, the contractor will develop a recovery plan that will be submitted and reviewed by CERN.

The list of NP and HP to be implemented during the various phases of the execution will be mutually agreed between CERN and the contractor. The minimum inspection and controls that will be performed during fabrication and installation are:

\begin{itemize}
\item Non-destructive test of welds
\item Helium leak tightness test
\item Cold test (during acceptance)
\item Pressure test
\item Cleanliness control
\item Dimensional control
\item Transport acceleration
\item Factory outlet inspection
\item CERN incoming inspection
\item Final position inspection
\item Positioning and layout control
\item Interfaces control
\item Hydraulic continuity control
\item Control of external supports
\end{itemize}


%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Detector monitoring and slow control}

\fixme{missing}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{QA/QC and testing space}
\section{Installation space and clean room}
\label{sec:quality:space}

All of the testing for the TPC components will be done inside the clean room or inside the cryostat. 

Once the APAs are moved into the clean room, a connectivity test will be performed to look for shorted or broken wires.  It will also be inspected visually for broken wires.  Tension tests will be performed on some fractions of the wires and the results will be compared to the ones taken at the production facility.

For the PDs, each PD will be unpacked and placed inside a full length dark box with a scanning VUV light source. This will be an identical test set up to the one used at the production facility.  Each test will take approximately 2 hours, which is the planned time for the installation and cabling of a PD into the APA.  

The CE modules will be delivered as an assembly.  The CE enclosure will have the electronics boards mounted inside and the internal cable from the harness connected and tested.  Each module will undergo an acceptance test when they are unpacked inside the clean room.  Once tested, they will be installed on the top of the APA frame from either a scaffold or a scissor lift located in the clean room.  A connectivity test will be performed on each module to ensure the electrical connections.  

After the APA has been fully integrated with the PD and CE, it will be moved via the rails in the clean room to the integrated cold testing stand.  This test stand, shown in Figure \fixme{6}, is a large insulated box that is light tight for PD testing and a Faraday shield for CE testing.  The test stand is shown with an APA inside and the end cover removed.  
%
\begin{cdrfigure}[short caption for table of figures]{label}{6 long caption that appears below picture}
%  \includegraphics[width=0.8\textwidth]{protoDUNE_cryostat.png}
\end{cdrfigure}
%
At the top of the box, there will be a crossing tube, similar to those in the cryostat, with a conflat fitting that will accept the warm – cold interface flange for the PD and CE cable connections.  The PD and CE cables will be routed and connected to their flanges, the APA will be moved inside and the end cover, that completes the Faraday cage, installed so that the integrated electronics testing can begin.  A series of warm tests will be performed.  This is described in \fixme{need to find... XXsectionXX}.  After the warm tests are complete, the inner volume of the enclosure will be purged with dry gas to reduce the moisture inside.  After this gas purge, the inner volume will be slowly cooled down using nitrogen gas to a temperature of approximately 100 K.  The rate of cooldown is to be less than 10 K/hr which is the same for the cryostat.  The cooldown system is being designed to maintain the inner volume near 100 K for approximately 48 hours.  The cold testing of this can be performed during the cooldown period, during these 48 hr and during the warmup.  After the testing is complete and the box has been purged of nitrogen with room air, it will be opened, the APA removed and the cables disconnected and secured for movement on the rail system.   

Each of the CPA panels will be visually inspected for damage to the resistive coating on the panels.  At the panels are assembled into a CPA module, electrical connections will be made and tested between the panels.  As the modules are mounted on the clean room rails, the modules will be electrically connected between the modules.  This connection will be tested in the clean room and when the CPAs are moved inside the cryostat to their final position.  

The FC assemblies will be visually inspected for damage as they are removed from their shipping containers.  The electrical connections between the divider chains will be tested.  Once attached to the CPA, an electrical connection between the CPA and FC must be made to carry the HV to the FC.  This will be tested in the clean room before moving the assembly into the cryostat. 





==> sciencetech.tex <==
%\chapter{sciencetech}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% \section{Overview}

The DUNE primary physics program focuses on long-baseline neutrino oscillation physics, nucleon decay and supernova burst and 
astro-physics \cite{dunecdr} and plans to employ a 40 kton LAr detector underground. The protoDUNE program will make 
measurements to significantly enhance the reach of DUNE in each of these areas. 
In addition, some protoDUNE measurements of hadronic interaction on Ar nuclei will be the first of their kind 
and hence are expected to be significant results in their own right. 





The DUNE sensitivity assumes a significant advance in a reduction of various sources of uncertainties. In table \ref{tab:DUNEsen} the list of collated sources of uncertainties compared with the lists for MINOS and T2K $\nu_e$ appearance analyses are presented. 
%
\begin{cdrtable}[DUNE goals are for the total normalization uncertainty on the $\nu_e$ appearance sample.] {ccccc} {DUNEsen} {DUNE goals are for the total normalization uncertainty on the $\nu_e$ appearance sample. The DUNE analysis will be a 3-flavor oscillation fit such that uncertainties correlated among the four FD samples will largely cancel \cite{cdr-vol-2}.}
Source of Uncertainty &  MINOS $\nu_e$ & T2K $\nu_e$ & Goal for DUNE $\nu_e$  \\ \toprowrule
 Beam Flux                        &  0.3\% & 3.2\%  &  2\%&  \\ \colhline
Interaction Model               & 2.7 \%  & 5.3\% & ~2\%  \\ \colhline
Energy Scale ($\nu_\mu$) &  3.5\% & included above  &  (2\%) included in  \\
					 &   &   &   5\% $\nu_\mu$ uncertainty  \\ \colhline
Energy Scale ($\nu_e$)     & 2.7\% & 2.5\% includes all FD effects &  2\% \\ \colhline
Fiducial Volume                 & 2.4\% & 1 \% & 1\%  \\ \colhline
Total Uncertainty                & 5.7\% & 6.8\% &  3.6\%  \\ \colhline
\end{cdrtable}
%
To achieve this reduction of uncertainties, a program of measurements is needed using various detectors. ProtoDUNE-SP will be particularly useful to measure detector effects with full-scale components as planned for the DUNE far detector and a long drift volume. 

While long-baseline physics studies are not sufficiently advanced to establish firm requirements on individual systematic parameters or detector effects the studies conducted to date indicate 
that energy scale measurements at the single particle level, efficiencies for calorimetry and background rejection, especially e-gamma 
separation are of particular interest. From the DUNE long-baseline physics perspective the goal of the protoDUNE measurements program 
should be the validation of detector simulations and measurement techniques such that these may be applied in the DUNE far detector environment.

Nucleon decay searches aim to discover or alternatively set a lower limit on the lifetime for specific decay processes. The lower limit 
on the partial lifetime is described by equation \ref{eqn:ndk_limit}
\begin{equation}
\tau/B = \frac{n_{p/n} \varepsilon M t} {N_{obs} - N_{backgr}} \,\,\, ,
\end{equation}
where  $\tau/B$ is the (lower limit on the) partial lifetime sensitivity (in yr).
On the right hand side of the equation
$n_{p/n}$ is the number of protons or neutrons per unit mass (in 1/kton ), $\varepsilon$ is the signal detection efficiency, $Mt$ is the detector exposure (in ton yr) and $N_{obs} - N_{backgr}$ is the (upper limit on the) number of signal events.

ProtoDUNE measurements will affect $\varepsilon$ and $N_{backgr}$ through 
particle identification performance and track and shower reconstruction performance measurements as well as
pion and kaon cross section measurements on Ar nuclei.
In addition, experimental data may 
help to refine the nucleon decay event selection in a LAr TPC which is equivalent to the DUNE far detector.

The study of atmospheric neutrinos in DUNE allows measurement of the mass hierarchy and oscillation parameters including 
a unitarity test by means of the tau neutrino appearance channel.  For atmospheric neutrino interactions simulation studies indicate that 
typically 1 to 5 hadrons are expected in the final state. While neutrino induced hadronic showers will be different from those produced by 
single particles in a test beam, the same nuclear models used for both types of interactions can be validated
Furthermore, reducing the angular and energy resolution for single hadrons and multi-particle hadronic systems is expected to lead 
to better mass hierarchy sensitivity. Measurements of and improvements to particle identification and pion and kaon interactions on Ar nuclei 
will improve the overall uncertainty of measurements relevant for atmospheric neutrinos.


For SNe neutrinos the relevant energy range of tens of MeV is significantly lower than what can be studied with charged particles at the H4 
beamline. However, stopping muons originating from the beam and from cosmics and associated Michel electrons will allow to study the 
detector response in the relevant energy range. In particular, the light yield of the photon detection system in response to Michel electrons 
will be of interest to evaluate PDS trigger efficiencies for SNe neutrinos. Stopping muons and Michel electrons also serve as low energy 
calibration sources and planned studies are described in that context in section \ref{sec:calibration}.


The following sections describe the planned studies sub-divided into measurements on the hadronic and electromagnetic systems
and measurements focused on the evaluation of event reconstruction and particle identification performance.

%%% For lepton energy resolution and energy scale uncertainty we would need to measure differences between particles and antiparticles and any nonlinear effects.  

%%% For hadronic energy resolution and energy scale uncertainty, there will be different contributions from different particles types (protons, neutrons, charged pions, neutral pions) in different portions of the neutrino spectrum. 
%%% One of the most important measurements will be a determination of the missing/undetected energy. 

%%%Below we provide a list of the main ProtoDUNE-SP studies that will be performed using charged particles from the beam and particles created by cosmic muons. The studies will inform us about the detector response to particles/tracks/showers that will be observed in the neutrino-induced events in the DUNE detectors. 


\section{Hadronic physics topics}
incoming primaries:  pion, proton: 1- few GeV

Accurate measurement of neutrino energy will require characterisation of both electromagnetic and hadronic showers. Reconstruction of hadron energy in these energy ranges will require knowledge of the fate (interact, decay, or stop) of the initiating hadron ($\pi^{+/-}$, $p$, or $K^{+/-}$).
For the case of interacting hadrons, the composition of secondaries
will need to be determined to characterise the response. 
These will include neutrals and particles that deposit energy electromagnetically ($\pi^o$, $\gamma$), as well as
secondary hadrons. The test beam with known incoming particle type and momentum will be used
to characterise interacting hadrons in this energy range.



\subsection{Energy scale}

for different shower complexities

%%%--- \item [Characterization of hadronic showers (high $p$) and topologies of hadronic interactions (low $p$).]



Figure~\ref{fig:hadronshwr} shows the fraction of true energy deposited by interacting protons with 1~GeV/c (left) and
3~GeV/c (right) incident momenta simulated using FLUKA particle transport code~\cite{fluka05}. 
Interacting protons (65\% of the 1~GeV/c sample) are selected.
For this study, visible energy is summed using hit information with corrections applied for the lifetime of the drift electrons (No attempt is made to correct for recombination effects or electromagnetic shower fractions). 
The resulting energy deposition in the two cases cannot be accurately characterized by an average shower calibration factor. MC simulations of outgoing particles, especially at low energies, must be checked and benchmarked against calibration data to avoid significant uncertainties from shower modeling. 

\begin{cdrfigure}[Fraction of true energy deposited by interacting protons of 1~GeV/c and
3~GeV/c]{hadronshwr}{Fraction of true energy deposited by interacting protons of 1~GeV/c (left) and
3~GeV/c (right) momenta simulated using FLUKA~\cite{fluka05}.}
\includegraphics[width=0.49\textwidth,height=5.0cm]{pr1GeV_v2a}
\includegraphics[width=0.49\textwidth,height=5.0cm]{pr3GeV_v2a}
\end{cdrfigure}


Pion showers at low energies will also be important both for determining the interacted neutrino energy and for modelling neutral current backgrounds resulting from $\pi^o$ content in showers. Significant differences in energy deposited in interactions initiated by $\pi^+$ versus $\pi^-$  are present up to momenta of an order of 1~GeV/c due to different final-state particles and interaction cross sections. This is illustrated in  Figure~\ref{fig:pionshwr}, which shows the differences in mean energy deposited (left) and width (right)  for interacting pions with momenta ranging from 0.2~GeV/c up to 5~GeV/c.
Resulting shower calibrations and reconstruction will differ; therefore each charge must be studied separately. This study will be performed if a low momenta run will take place.  

\begin{cdrfigure}[Differences in mean energy deposited and width of visible energy, 
 $\pi^+$ versus $\pi^-$]{pionshwr}{Differences in mean energy deposited (left) and width of visible energy (right) 
for interacting $\pi^+$ versus $\pi^-$ ranging from 0.2~GeV/c up to 5~GeV/c. }
\includegraphics[width=0.49\textwidth,height=6.0cm]{pipimean_ticks1}
\includegraphics[width=0.49\textwidth,height=6.0cm]{pipisigma_ticks1}
\end{cdrfigure}




\paragraph{Missing energies}
	     
	     The measured energy deposition for various particles and its dependence on the direction of the particle will be used to tune
MC simulations and allow improvements to the reconstruction of neutrino energy and interaction topologies. 
Measurements of the response to charged particles and photons with the protoDUNE-SP will extend and be complementary to
measurements made with other smaller detectors, such as LArIAT \cite{lariat}.
 LAr TPC enables the use different energy reconstruction methods. 
 %In particular, in LAr TPC we can infer $E_\nu$ from what we observe in the final state. 
 ArgoNeuT neutrino energy reconstruction method included estimates of missing/invisible energy, and important part of the improved neutrino energy reconstruction included the measurement of neutrons. 
 Precise and unbiased neutrino energy reconstruction is especially important for reducing systematics in precision neutrino oscillation experiments. The systematic uncertainty which creates a bias in neutrino energy measurement  affects the ability to precisely measure oscillation parameters.  The inclusion of neutrons in the estimation of neutrino energy improves energy resolution from 14\% to 3\%
 \fixme{need reference}.  
 Due to its large size protoDUNE-SP has the ability to measure protons that are created via the neutron-proton charge exchange process.
 Hence it allows to validate the accuracy of missing energy fractions as predicted by MC simulations and thereby improve the uncertainty on the 
 energy bias.

	     
\subsection{Studies of e.m. fractions}

 (as function of primary hadron energy)
	
	
\subsection{Multiplicities in hadronic interactions}
 (pi0 and others)

\subsection{Shower topologies}


\subsection{Shower development}
  (energy deposition mechanisms)\\
	  Ñ> verification of MC models

	
\subsection{Cross section measurements}
 (exclusive + total hadronic)\\
		(absorption, charge exchange, inelastic, elastic, É)\\

Detailed knowledge of pion-nucleus cross sections in the sub-GeV energy range is required to tune generators~\cite{genie} to model event visible energy accurately. 
Existing data used to tune the models cover limited energies ($<$200~MeV) and are primarily on lighter target nuclei~\cite{fsirev}.
The requested $\pi^+$ and $\pi^-$ samples will allow new data samples for measuring
exclusive final state processes of $\pi^+$ and $\pi^-$ over the full relevant \fixme{quantify} energy range and specifically on argon nuclei. 
The H4 beam line will allow to collect $\pi^+$ and $\pi^-$ data with momenta above\,1~GeV/c.  
Synergies with the LArIAT experiment will be explored to investigate agreement within the overlapping energy region.  A high-statistics sample of charged particles will allow precise measurements of charged mesons' interaction cross sections and particularly various exclusive channels.


\paragraph{Pion interactions}
		
		Final state pions are produced copiously in neutrino interactions in the energy range for the DUNE beam  and contribute 
substantially to the total visible energy in the interaction.
Pions can re-interact either in the nuclear medium or after emerging from the target nucleus
and significantly change the visible energy deposited in the event. 
The importance of modeling final-state pion interactions on reconstructed neutrino energy has been recently demonstrated in the NuMI, and Booster beam energy ranges~\cite{miniboonefsi, minervafsi}. The results from Minerva and MiniBoone are in tension and even more sophisticated final state interaction models cannot resolve the disagreement. 



\paragraph{Resonance production}
	 
\subsection{Pi-zero production model tests}

\subsection{Kaon interactions}
 rare in beam line but numerous from pion interactions in side detector\\ 
	       Ñ> kaon decay\\
		==> p-decay sensitivities\\

%%%--- kaon interaction cross section to remove proton decay backgrounds

The DUNE experiment in the deep underground location will seek to detect several modes of proton decay.
%In particular, a first ever LAr detector 

This first-ever LAr detector of this scale underground will primarily improve sensitivity to proton decays with final state kaons such as  ${p \rightarrow K^+ \overline{\nu}}$. 
Sensitivity to this process is studied in~\cite{bueno}. $K^+$ detection efficiency is estimated to be $>$97\% in the
appropriate momentum range (500-800 MeV/c). The kaon samples needed for this study might not be available in the H4 beam line, as most of the kaons will decay before reaching the protoDUNE detector. 

To provide the needed 2000 stopping $K^+$ track samples for the PID studies, a sample of 13k beam kaons with 1~GeV/c momentum must be obtained (Only 15\% of $K^+$ stop at 1~GeV/c.), which will likely be difficult in this beam line. 
A sizable sample of protons ($\sim 10^6$) is also needed. This will allow a study of the possible background contributions to $p \rightarrow K^+ \overline{\nu}$ to quantify the probability of an interacting proton being misidentified as stopping kaon. A proton interaction that produces neutrals and one charged pion 
(that is misidentified or subsequently decays to $\mu$) can fake the final-state kaon signal.




\section{Electromagnetic physics topics}

%Electromagnetic showers are relatively well-understood and can be used to understand the detector response better. 
The beam of electrons will be studied at various energies to characterize the induced showers.

Decays of neutral pions induced in the interactions of hadrons in the beam at one to few GeV/c momentum
will be used as a source of photons producing electromagnetic showers at a broad range of angular orientations.
This sample will be used to validate techniques for electromagnetic showers separation from the hadronic
component of the event. Such techniques are a prerequisite for the use of the generic EM shower reconstruction
algorithms (see section ~\ref{sec:larsoftreco}), and in particular for studies of energy scale calibration
based on neutral pion invariant mass reconstruction. Also, hadronic shower energy estimation, as mentioned
in the previous section, requires splitting between electromagnetic showers and hadronic tracks. Finally,
test beam event topologies with $\pi^0$ production are similar to those expected in neutrino events, and
will be studied as described in the following section.


	\subsection{Electron shower}

		\paragraph{Energy resolution}
		 (at higher energies)

		\paragraph{Energy scale}

	\subsection{e/gamma separation}
	
	The search for a CP violation phase using $\nu_e$ appearance 
in a $\nu_\mu$ beam requires good electron/photon separation.
Backgrounds originating from photons produced primarily from final state $\pi^0$'s must be identified and removed from the signal
electron sample. 

High-energy photons can undergo two processes: pair production and Compton scattering. 
The dominant process for photons with energies of several hundred MeV or more is 
e$^+$ e$^-$ pair production.
For this process e/$\gamma$ discrimination can be achieved using the beginning of the electromagnetic shower, where a single MIP is characteristic of electron energy deposition, while two MIPs would be consistent with e$^+$ e$^-$ pair production. 


\begin{cdrfigure}[Photon background rejection versus electron identification efficiency for various energies]{egam}{Photon background rejection versus electron identification efficiency for various energies( 100 MeV - 5 GeV for photons and 100 MeV - 2 GeV for electrons), calculated for and normalized to samples which pass the reconstruction.  The simulation was performed in APA design configuration (4.67-mm wire pitch, induction wires at $\pm$35.7$^{\circ}$ w.r.t. collection wires).}
\includegraphics[width=0.5\textwidth,height=6.0cm]{egammaeffbkg}
\end{cdrfigure}


Electron-photon separation has been studied in LArTPCs  detectors that collected data in recent years (ICARUS~\cite{icarus_eg} and ArgoNeuT~\cite{argoneut_eg}).

Figure~\ref{fig:egam} shows estimated photon background rejection versus electron identification efficiency using simulated isotropic electron and photon event samples with the DUNE APA geometry configuration (4.67-mm wire pitch,
induction wires at $\pm$35.7$^{\circ}$ w.r.t. collection wires).~\cite{dunecdr}. The study was performed on the
simulation of isolated particles to separate from the present state of the art of pattern recognition algorithms
and their inefficiencies. Instead, the unavoidable features, such as an overlay of signals from multiple tracks in the
interaction vertex region, was mimicked with the parameterized subtraction of information from the initial part of
simulated cascades.

The results are found to be mildly dependent on incoming particle energy in the range of interest. 

Pure samples of electrons and photons in the sub-GeV energy range would be required to tune the separation algorithms and to measure detector-dependent electron-photon separation efficiency and purity. 
Such an idealistic conditions cannot be easily achieved with the test beam, but charged pion interactions might be very well studied to evaluate performance of the background rejection based on the observation of double m.i.p. and (or) photon-induced cascade displacement from
the interaction vertex.

	
	\subsection{Charge identification via muon capture}

With non-magnetized LArTPC detectors, it is not possible to determine particle charge on an event-by-event basis. Therefore, a statistical separation that makes use of differences in muon versus antimuon capture cross sections and lifetime will be investigated.
About 99.9\% of $\mu^-$'s are expected to be captured on argon, compared to essentially all $\mu^+$ to decay ~\cite{stopmu}.
Charge-sign tagged $\nu_\mu$ samples, which predict differences in the particle and antiparticle survival probabilities, may be useful for constraining exotic possibilities, such as non-standard neutrino interactions. 
A well-developed muon tagging would enhance the MH studies for the atmospheric neutrinos. 


\section{Evaluation of event reconstruction and particle identification performance}

	\subsection{Reconstruction algorithm performance test}

		\paragraph{Energy dependency}
		\paragraph{Efficiencies}

	\subsection{Particle Identification}
	
	Information on a range and charge deposition for stopping charged-particles can be used to identify particle type as well as measure kinetic energy accurately. Figure~\ref{fig:resrange}  (left) shows track energy loss per unit length \footnote{Signal attenuation due to recombination effect is not corrected for the PID purpose since it is a deterministic transformation which does not add measurement information.} $dQ/dx$ as a function of residual track range for simulated muon, pion, and proton particle tracks. The sequence of $dQ/dx$ versus residual range reconstructed for a particle track is used as input to PID algorithms ~\cite{nn_pid,rd_pid} to evaluate each particle hypothesis.

Figure~\ref{fig:resrange} (right) shows the distribution of reconstructed $dQ/dx$ in a narrow bin at a residual range of 6($\pm$1)cm to illustrate the scale of difference between particle types. Proton band is well separated from pion and muon bands, while pion and muon bands are almost overlapping which is challenging for the efficient separation via ionization density differences. 
Simulation is performed with LArSoft framework using ProtoDUNE-SP geometry including the beam orientation and GEANT4 based simulation of particle transport through LAr. Parameterization of the detector response is implemented according to the scheme existing in the LArSoft framework, with a dedicated setup for ProtoDUNE-SP conditions. Pattern recognition and 3D reconstruction are performed with Line Cluster and Projection Matching algorithms (one of standard reconstruction schemes currently used for ProtoDUNE).

The PID efficiency and purity depend on a number of factors, such as the detector configuration, geometry and reconstruction algorithms. PID results on data, especially for pion/muon separation, may be significantly different if e.g. electronics noise assumed in the detector response simulation is not reproducing features of the DUNE readout chain or if signal processing and reconstruction algorithms are updated. It is, therefore, important to test entire PID scheme in a prototype detector data, using the presence of all detector effects to improve models used in both simulation and reconstruction. Event samples that include an adequate number of stopping particles for each species
(muon, pions, protons and kaons) are included in the particle summary request to perform tests of PID algorithms and Bethe-Bloch calibration measurements.

\begin{cdrfigure}[ProtoDUNE-SP simulated track $dQ/dx$]{resrange}{ProtoDUNE-SP Simulated track $dQ/dx$ as a function of residual range for muons, pions, protons and kaons, used as training data in a neutral-net-based PID algorithm (left). Distribution of $dQ/dx$ for each particle type for a bin with residual range 
6($\pm$1)~cm (right). The small difference between muon and pion PID is illustrated.}
\includegraphics[width=0.53\textwidth,height=6.0cm]{dEdxprmupi}
\includegraphics[width=0.46\textwidth,height=6.0cm]{dEdxprmupienbin}
\end{cdrfigure}


		\paragraph{Stopping particles}

		\paragraph{Low energy}

		\paragraph{e/gamma separation}
 	also have this under em physics already ...




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Detector engineering validation}

One of the primary goals of the ProtoDUNE-SP experiment is to validate the engineering design of the elements proposed for the 10 kt DUNE single-phase detector. ProtoDUNE-SP is designed so that it will provide information on the actual far detector performance in as close a possible a configuration to the actual far detector layout as possible given the practical considerations imposed by time, space, and cost. To achieve this the cold components are wherever possible identical to the components proposed for the far detector. 

As an example the APA modules are full-scale pre-production modules for the far detector. The full-scale APA modules have 20 front end readout board instrumenting each and 10 integrated photon detector paddles. The ground connections between the electronics, the APA mechanical structure, the photon detectors, and the detector support structure will be as proposed for DUNE SP detector. ProtoDUNE-SP is instrumented with three APAs along each wall which will test that there is no cross talk between the middle APA and the neighboring ones. However, there are some practical limitations which required compromise in the ProtoDUNE design. The far detector is designed with a 12 m high TPC based on a two APA high layout where the bottom APA is hung from the top. Given the space available and generally the cost of the cryogenic infrastructure it is not practical to have a 12 m high test experiment. For these reasons ProtoDUNE-SP is designed with a single APA high TPC. The collaboration will test separately the mechanical process of installing the two APA detector configuration along with the related cabling.

The readout electronics is designed based on the far detector cryogenic front end pre-amp/shaper chip and ADC.  The dedicated ASIC for serializing the data and providing a 1GB/s link is not yet available so an FPGA emulating its functionality will be used and is mounted on a dedicated mezzanine board. It should be pointed out that all the analog components, the conversion to digital and the grounding/power distribution for the final electronics can be tested in this configuration. 

ProtoDUNE-SP will be the largest experiment to take data with the cold electronics allowing high statistic detailed studies of the performance. In the event further optimization of the ASICs are required based on the ProtoDUNE-SP findings, this can be implemented before production start in 2020. As there is no charge amplification in the liquid in the Single-Phase detector, the electronics must be extremely sensitive which makes the grounding and shielding critical. The ProtDUNE-SP experiment is designed to be as close to the far detector grounding as practical. The building ground in ENH1 with all the rebar in the concrete floor interconnected and then this network connected to the building ground bus should provide a fairly good ground for ProtoDUNE. The cryostat itself is isolated from the building ground and all the mechanical/electrical connections have dielectric breaks. At the far site the detector is a mile underground in a very dry mine so one expects better isolation from the environment, but the ProtoDUNE will test the ground isolation and shielding under conservative conditions.

The field cage and cathode planes are full-scale prototypes of the final far detector elements. As the ProtoDUNE-SP detector is designed with full-scale field cages the maximum drift distance and corresponding high voltage will be the same as planned for the far detector. This allows ProtoDUNE to use the same high voltage feed thru as DUNE-SP and the drift field configuration that is planned for the far detector. The cryostat dimensions are selected to be the same as the Dual-Phase cryostat in order to only need to design one cryostat and cryogenic system. In order to fit in the cryostat the wall to cathode plane distance is slightly smaller than in the far detector making this setup a conservative test of the HV design. The ground planes above and below the detector make the actual mechanical geometry inside the cryostat on the top and bottom irrelevant for issues related to high voltage. This preserves the freedom to tailor the far detector cryogenics system as needed to optimize the purification without compromising the validity of the ProtoDUNE test. 

Testing these components under nominal operating conditions is extremely important as this is the first instance of LArTPCs operating with a resistive cathode or the field cage construction with metal profiles and fiberglass I-beam support. In the event ProtoDUNE-SP wishes a second run with a shorter drift distance in order to reduce the effects of space charge the FC can be shortened to 2.5 m maximum drift distance.

ProtoDUNE offers a unique platform to validate and possibly optimize the cryogenic design for DUNE. The DUNE 35t prototype was the first membrane cryostat to achieve high purity operation, but it was limited to roughly 3 ms $e^-lifetime$. This is substantially worse than the MicroBooNE experiment's  $\sim$10 ms or the lifetimes seen at ICARUS at the end of its last run. 

There are several possible causes for a shorter electron lifetime.  A third of the 35t cryostat roof is covered with a hatch that is not insulated but designed with radiation shields. As the dominant source of contamination is the transfer of impurities in the gas ullage to the liquid, the gas circulation in the ullage and the impact of the hatch are important factors in the cryostat/cryogenics design. The purity monitors inside the 35t cryostat also indicated that the liquid was not well mixed with substantially higher purity at the bottom of the cryostat indicating that the liquid feed and temperature need to be optimized.  

The ProtoDUNE-SP cryostat design does not have a hatch for the detector installation instead a temporary construction opening (TCO) is used (similar to the Dual-Phase cryostat). The Single-Phase detector moved to this option after the difficulties encountered in the mechanical design of the hatch for the 1x1x3 cryostat and based on the recommendations from the cryostat design team.  This will also eliminate one potential source of contamination to the liquid argon. It should be pointed out that with a 3 ms lifetime and a 2.25 ms maximum drift time roughly half the charge generated near the cathode is lost before it reaches the anode. Efforts to improve the electron lifetime will improve the detector performance.  Cryogenic design improvements are that the Proto-DUNE SP detector will not have a hatch in the ullage, all cryostat penetrations will be designed with gas purge to prevent contaminates from migrating from warm surfaces to the ullage volume, and the cryostat/cryogenic system will be modeled to understand the liquid and gas flows inside the cryostat. ProtoDUNE-SP will provide an excellent test bed to prove the cryogenic design for DUNE. 

The installation process has many similarities to the far detector installation but also many differences. Both installation plans now call for inserting the equipment through a TCO. ProtoDUNE-SP will prototype the tooling and procedures for transporting an APA and transferring to to a suspended rail system. Similarly the assembly and transport of the cathode planes and top/bottom field cages will be developed. What will not be tested is the hanging of one APA from the other and the difference in moving a 12 m stack instead of one 6 m module. Likewise the CPA is only 6 m tall instead of 12 m. One major change in the installation was forced by the need to install the end walls with the TCO closure and the beam interface. Due to the tight space inside the cryostat the rail structure on which the detector is hung will most likely be different for the final detector. However the experience in installing the ProtoDUNE-SP detector will be invaluable in planning the DUNE far detector installation. 

Finally one significant difference between the ProtoDUNE-SP detector and the single-phase far detector is the integration of the test beam. This requires a penetration into the cryostat and a liquid argon displacement plug bridging the gap between the membrane cryostat wall and the detector field cage. As this element bridges the high voltage careful design is required. To insure that the displacement plug does not compromise the ProtoDUNE-SP operation a dedicated HV test at FNAL is planned which will test the final beam plug in the exact field configuration planned for ProtoDUNE.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%---\section{Installation validation}






==> summary.tex <==
%\chapter{summary}

This is the summary.  Write me.


==> tpc-signal-extraction.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{TPC Charge Extraction}
\label{sec:tpc-signal-calibration}

In Section~\ref{sec:tpc_signal_formation}, the signal formation in a single-phase LAr TPC
is described. This section describes the procedure of the TPC 
charge extraction. As shown in Figure~\ref{fig:signal_formation}, the 
goal of TPC charge extraction is to recover the number of ionized 
electrons from the digitized TPC signal. 

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Deconvolution Technique}\label{sec:decon}
\label{sec:decon-tech}
Deconvolution is a mathematical technique to extract the \textit{underlying true signal}
$S(t)$ from a \textit{measured signal} $M(t_0)$. The deconvolution technique 
was introduced to LArTPC signal processing in LarSoft in the context of ArgoNEUT data analysis~\cite{bruce}. 
The goal of the deconvolution is 
to ``remove'' the field and electronics response functions from the measured 
signal to recover the underlying true number of ionizing electrons.~\footnote{Strictly speaking,
the deconvolution replaces the bipolar response function with a unipolar smearing
function.} This technique has the advantage of being robust and fast and is an 
essential step in the overall charge extraction process. 

The measured signal is modeled as a convolution integral over the true 
signal $S(t)$ and a given detector \textit{response function} $R(t,t_0)$ which gives the
instantaneous portion of the measured signal at some time $t_0$ due to
an element of the true signal at time $t$.
\begin{equation}\label{eq:decon_1}
M(t_0) = \int_{-\infty}^{\infty}  R(t,t_0) \cdot S(t) \cdot dt.
\end{equation}
If the detector response function only depends on the relative time 
difference between $t$ and $t_0$, the above equation can be solved by 
doing a Fourier transformation on both sides of the equation:
\begin{equation}
M(\omega) = R(\omega) \cdot S(\omega), 
\end{equation}
where $\omega$ is the frequency. In this case, we can derive the signal in the 
frequency domain by taking the ratio of the measured signal and the assumed
response function:
\begin{equation}\label{eq:decon_2}
S(\omega) = \frac{M(\omega)}{R(\omega)}.
\end{equation}
The true underlying signal in the time domain can then be obtained by applying the 
inverse Fourier transformation from the frequency domain. 

The Shockley-Ramo response function $R(\omega)$ does not address
contributions to the measured signal which are due to real world
sources of electrical \textit{noise} from thermal and unwanted transmitting
sources or due to the approximation in the digitization.
Such contributions to $M(\omega)$ will not be ``divided out'' by the deconvolution.
Worse, because the response function becomes small (see Section~\ref{sec:decon-2D-ind}) %below) 
at low 
frequencies for the induction planes and at high frequencies for all
planes, the noise components in these frequencies will become
enhanced by the deconvolution.

To address the problem of noise, a \textit{filter function} $F(\omega)$ is
introduced.  Its purpose is to attenuate the problematic noise.  The
addition of this function can be considered an augmentation to the
response function, which may in any case be chosen freely as it is a model.  
The two functions are kept distinct for clarity in the notation here.
Equation~\ref{eq:decon_2} is then updated to become
\begin{equation}\label{eq:decon_filt}
S(\omega) = \frac{M(\omega)}{R(\omega)} \cdot F(\omega).
\end{equation}
With a suitable noise model, an improved estimator for the signal
$S(t)$ in the time domain can then be found by applying an inverse Fourier 
transform to $S(\omega)$.  Essentially, the deconvolution replaces the field and 
electronics response function with the filter response function. The 
advantage of this procedure shows up on the induction plane where the irregular bipolar 
field response function is replaced by a regular unipolar response function through
the inclusion of the software filter. 


%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Importance of 2D Deconvolution for Induction Planes}
\label{sec:decon-2D-ind}

The 1D deconvolution procedure described in Section~\ref{sec:decon-tech} %the previous section 
works well in dealing with signal in the collection wire plane, but is not 
optimal when applied to signals in the induction wire planes. 
As described in Section~\ref{sec:tpc_signal_formation}, the induction plane wire 
signal receives contributions not only from ionization charge 
passing by the wire of interest, but also from ionization charge drifting in 
nearby wire boundaries. In addition, within the boundary of the wire of 
interest, the value of the field response function varies appreciably 
 so at small scales the location of the drifting charge relative to the wire 
is important. In this case, Equation~\ref{eq:decon_1} would naturally expand to 
\begin{equation}\label{eq:decon_2d_1}
M_i(t_0) = \int_{-\infty}^{\infty} \left( R_0 \cdot (t-t_0) \cdot S_i(t) + 
R_1 \cdot (t-t_0) \cdot S_{i+1} (t) + ...\right) \cdot dt,
\end{equation}
where $M_i$ represents the measured signal from wire $i$.  $S_i$ and
$S_{i+1}$ represents the true signal in the boundaries of wire $i$ and
its next neighbor, respectively.
$R_0$ represents the average response function for an ionization
charge passing through the region for the wire of interest.
Similarly, $R_1$ represents the average response function for an
ionization charge drifting through the next adjacent wire region. One can
easily expand this definition to some number of neighbors by introducing terms up 
to $R_{n-1}$.

If one applies a Fourier transformation on both sides of Equation~\ref{eq:decon_2d_1},
we have:
\begin{equation}\label{eq:decon_2d_2}
M_i(\omega) = R_0(\omega) \cdot S_i(\omega) + R_1(\omega) \cdot S_{i+1} (\omega) + ...,
\end{equation} 
which can be written in a matrix notation as:
\begin{equation}
\begin{pmatrix}
    M_1(\omega)\\
    M_2(\omega)\\
    \vdots\\
    M_{n-1}(\omega)\\
    M_{n}(\omega)
\end{pmatrix}
=
\begin{pmatrix}
R_0(\omega) & R_1(\omega) & \ldots & R_{n-2}(\omega) & R_{n-1}(\omega) \\
R_1(\omega) & R_0(\omega) & \ldots & R_{n-3}(\omega) & R_{n-2}(\omega) \\
    \vdots  & \vdots      & \ddots & \vdots          & \vdots \\
    R_{n-2}(\omega) & R_{n-3}(\omega) & \ldots & R_0(\omega) & R_1(\omega) \\
    R_{n-1}(\omega) & R_{n-2}(\omega) & \ldots & R_1(\omega) & R_0(\omega) \\
\end{pmatrix}
\cdot
\begin{pmatrix}
    S_1(\omega)\\
    S_2(\omega)\\
    \vdots\\
    S_{n-1}(\omega)\\
    S_{n}(\omega)
\end{pmatrix}
\label{eq:matrix_expansion}
\end{equation}
Assuming the response functions (i.e., the matrix $R$) are known, the 
problem converts into deducing the vector of $S$ with the measured signal $M$. 
%
This can be achieved by inverting the matrix $R$. In practice and away
from plane edges the matrix $R$ is taken to be symmetric and its
inversion can again be achieved by FFT.
%
As this expands the 1D deconvolution (with respect to the time axis)
into a 2D deconvolution (with respect to both the time and wire
axes), the filter function must be expanded in a similar fashion to cover
both time and wire dimensions.

A comment on the limitation (or approximation) 
assumed in the 2D deconvolution is needed. As shown in Equation~\ref{eq:decon_2d_1}, the 
average response functions are used in describing the measured signal. These 
ignore the detailed position dependence of the response function. 
This approximation ignores the fine-grained but clear position
dependence in the calculated weighting fields.
However, since the signal from any given wire can only be measured as
a function of time, there is no additional information to be used to
resolve the ionization electron distributions within a wire boundary.
This technique can in principle be improved to include the position-dependent
response once the local ionization charge distribution is roughly reconstructed. 

%%%%%%%%%%%%%%%%%%%%%%%%

%\fixme{sections 3.4.3 - 3.4.7 would benefit from a more focused description; as written it is a bit of a laundry list}
\subsection{Additional Challenges in Deconvolution}


The 1D and 2D deconvolution procedures provide a robust method to extract the ionization
electrons for the collection and induction planes, respectively. 
%
While working well for the collection plane, the procedure is still not optimal 
for the induction plane due to the nature of the induction plane signal. 
Figure~\ref{fig:induction_field} shows the field response as simulated with Garfield~\cite{garfield}
for induction and collection wire planes and point ionization
electrons. While the field response for the collection wire plane is unipolar, the field 
response for the induction wire plane is bipolar. 
%
\begin{cdrfigure}[Simulated field response functions in the time and frequency domains]{induction_field}{(left) Simulated field response functions for induction (black and red) and 
collection (blue) wires are shown in the time domain. (right) The same are shown in 
the frequency domain.}
\includegraphics[width=0.95\textwidth]{induction_field_response.png}
\end{cdrfigure}
%
The early, negative half corresponds to the ionization electron moving
towards the wire plane and the late, positive half corresponds
to the ionization electron moving away.
%
The integration of the field response function is close to zero
as the bias wire voltages are applied such that that none of the ionization electrons are
collected. The right panel of Figure~\ref{fig:induction_field} shows the 
frequency components of the field response. 
%
Since an induction plane field response has a bipolar shape in the time domain 
there is a corresponding suppression at low frequency in the frequency 
domain. At zero frequency, the frequency component essentially gives the 
integration of field response function over time and thus should be near 
zero (again, because no charge is collected).


The suppression of the induction field response at low frequency is problematic for the
proposed deconvolution procedure. First,  the measured signal contains the electronic noise, 
which usually increases at low frequency (the so-called 1/f noise). Therefore, as shown in 
Equation~\eqref{eq:decon_filt}, the low-frequency noise will be amplified in the deconvolution 
process, since the denominator (i.e., the induction field response) is generally small at 
low frequency. This can be seen clearly in Figure~\ref{fig:decon_example}, where the low-frequency noise
is significant. The large low-frequency noise would lead to large uncertainty 
in the charge estimation, and needs to be dealt with.  

\begin{cdrfigure}[Example of deconvoluted spectrum for the induction plane (simulation)]{decon_example}{Example of deconvoluted spectrum for the induction plane (simulation).}
\includegraphics[width=0.6\textwidth]{decon_example.png}
\end{cdrfigure}


In Equation~\eqref{eq:decon_filt}, a frequency-domain  filter function is introduced 
to suppress the numerical instability caused by the presence of noise. One can imagine using % to use 
this software filter to suppress the electronic noise at low frequency. 
However, such a filter is not acceptable due to the large distortion which it introduces to the signal.
To illustrate this point, recall that the software filter is effectively a smearing function. 
Figure~\ref{fig:low_f_filter} shows an illustrative true signal (left), its convolution 
with a low-frequency filter (middle), and the low-frequency filter itself (right). 
It is obvious that the signal is strongly distorted due to the application of the 
low-frequency software filter. 

\begin{cdrfigure}[Impact of the low-frequency filter]{low_f_filter}{The impact of the low-frequency filter (right). The unit of the $x$-axis 
is MHz.  The true signal and the convoluted signal are shown in the left and
middle panels, respectively. A time tick corresponds to 0.5 $\mu s$.}
\includegraphics[width=0.95\textwidth]{low_freq.png}
\end{cdrfigure}

In order to deal with this problem, we turn to using two techniques in the time domain: 
\textit{region of interest (ROI)} and \textit{adaptive baseline (AB)}. The ROI technique~\cite{roi}
was proposed in the context of reducing data size and speeding up the 
deconvolution process. At the same time, the ROI technique can %also 
be used to 
suppress the low-frequency noise. In order to recognize this point, consider
a time window with $N$ time ticks.  For ProtoDUNE-SP, this would be a window of 
$N\times0.5\mu\mbox{s}$. The highest frequency that can be resolved with such 
sampling would be 1~MHz. The first discrete frequency above zero would be $2/N$ MHz, 
and no result within the ROI can be sensitive to any noise components below this 
frequency.  Therefore, if we can identify the signal region and create a ROI to 
cover the signal, we can naturally suppress the low-frequency noises. 

The adaptive baseline (AB) technique~\cite{ab} was introduced  
in the context of 
dealing with the ASIC saturation observed in MicroBooNE. The AB is essentially a 
local baseline calculated in a given a ROI. However, instead of a simple average of 
the baseline at the start and end points of a ROI, a linear interpolation is used to 
correct the baseline. Given the two constraints (start and end points of the ROI), 
the linear interpolation with two degrees of freedom is the best that one can achieve 
to remove bias in the baseline. \\
%
In Section~\ref{sec:decon-frf-calc} %the following, 
we describe various techniques 
used in the charge extraction.

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Calculation of Field Response Function}
\label{sec:decon-frf-calc}

The field response is calculated with Garfield~\cite{garfield} in a 22-cm (along the 
field direction) $\times$ 30-cm (along the wire plane direction) region in 2D.  
In the drift direction, the grid plane is labeled as G, the two induction %planes 
wire planes are labeled U and V, and the collection plane is W.  The spacing between the wire 
planes is 4.76~mm. The bias voltages of-665 V, -370 V, 0 V, and +820 V for the G, U, V, and 
W planes, respectively, are configured according the operating conditions that ensure near 100\%
transmission of ionization electrons through the first two induction planes.  
A total of 101 wires of 150 $\mu$m diameter and with a pitch of 4.667 (4.79 for collection) mm make up
 each wire plane. 
    A ground plane is placed 1~cm behind the W plane.  The nominal drift
    field is uniform and has a magnitude of 500~V/cm. The electron drift velocity as a function of
    electric field is taken from measurements~\cite{Li:2015rqa,lar_property}
    instead of using the default velocity table contained in~\cite{garfield}. % Garfield. 
    The electron diffusion is turned off in the simulation. 
    For an 
    electron drift that starts from an arbitrary position within the ROI, the field response can
    be calculated for each individual wire in the form of induction currents 
    (U and V planes) or collection currents (W plane) as a function of time.

\begin{cdrfigure}[Description of the Garfield 2D simulation of field response 
functions]{garfield_2d}{Illustration of calculation of field response funciton with Garfield 2D simulation.
Top left panel shows the simulation for a track traveling parallel to the wire plane. Top right panel
shows the simulation for a single electron. The orange lines represent the track trajectory of ionization
electrons. See text for detailed description.}
  \includegraphics[width=0.95\textwidth]{Garfield_simu.png}
\end{cdrfigure}
%\fixme{Figure~\ref{fig:garfield_2d} needs a more descriptive caption}
    
    
    Figure~\ref{fig:garfield_2d} shows the configuration used in the Garfield 2D simulation.
The Garfield-simulated response functions are shown in Figure~\ref{fig:overall_response}.
 The average response function for single electrons within a wire region 
is calculated for the closest wire $R_0$, next adjacent wire $R_1$, and so on. The U and 
V plane response functions are shown in the middle and right panel of 
Figure~\ref{fig:overall_response}, respectively.  For induction wire planes, these response 
functions are reasonably balanced, as expected.




\begin{cdrfigure}[Overall response functions]{overall_response}{The overall response functions, i.e., %which is 
the convolution of the
electronics response function (14 mV/fC gain and 2 $\mu$s shaping time) 
and the field response. The response functions for the closest wire $R_0$ as defined in 
Eq.~\eqref{eq:matrix_expansion}, the next adajacent wire $R_1$, and so on, are plotted.
}
\includegraphics[width=0.95\textwidth]{dune_field_res.pdf}
\end{cdrfigure}
%\fixme{This needs more description in the caption.}

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Choice of Software Filter}

Two types of filters are selected and implemented.  The first, inspired by the Wiener filter,  
 is modified to not suppress low-frequency components.  The second is the 
Gaussian filter. While the first one is optimized independently for each wire plane to produce a 
high signal-to-noise ratio, the second one is optimized for the three planes as a group % and same to all the planes 
to correctly estimate the charge which is independently measured on each  plane. %of the three planes.  
This latter is important if all three planes are used for energy measurement 
and is critical for proper application of the Wire-Cell imaging technique~\cite{wire-cell}.  
In this section, we describe the selection process that resulted in %choice on 
these software filters.

The standard Wiener noise filter~\cite{wiener} is constructed from the expected 
signal $S(\omega)$ and noise $N(\omega)$ frequency spectra:
\begin{equation}
F(\omega) = \frac{S^2(\omega)}{S^2(\omega) + N^2(\omega)}.
\end{equation}
With this construction, the Wiener filter is expected to achieve the best signal-to-noise ratio. 
However, applying the Wiener filter to TPC signal processing is problematic. 
First, in a LArTPC, the TPC signal $S(\omega)$ varies substantially
depending on the exact nature of the event topology.
Second, the electronic noise spectrum is a function of the time window
over which it is observed. A longer time window allows for observation
of more low-frequency noise components.
Third, the induction wire signal spectrum is small at low frequency
and so would be its Wiener filter output.  As discussed previously, 
a software filter with low-frequency suppression leads to large distortions 
of the signal and is thus not ideal.  

The functional form of the software filter is chosen as:
\begin{equation}
F(\omega) = 
\begin{cases}
e^{- \frac{1}{2} \cdot \left( \frac{\omega}{a} \right)^b} &  \omega >0 \\
0 &  \omega = 0, \\
\end{cases}
\end{equation}
where $a$ and $b$ are two free parameters.  Note, $b=2$ is basically the Gaussian filter. 
The filter is explicitly zero at $\omega = 0$ in order to remove the DC component in the 
deconvoluted signal. This removes information about the baseline;  a new baseline is 
calculated and restored for the waveform after deconvolution. The above functional form 
of the filter has another advantageous property:
\begin{equation}
lim_{\omega \rightarrow 0} F(\omega) = 1.
\end{equation}
which means the integral of the smearing function is unity, which does not introduce any
extra factor in the overall normalization. The free parameters $a$ and $b$ in the above 
form are determined by matching the tail of the Wiener filter at its high-frequency side. 
An example of a software filter is shown in Figure~\ref{fig:soft_filter_1}. 

\begin{cdrfigure}[Wiener-inspired filter and Gaussian filter used in the 2D deconvolution]{soft_filter_1}{
The Wiener-inspired filter and Gaussian filter used in the 2D deconvolution are shown on 
the left (right) panel for the time (frequency) domain. A bin in the time domain plot represents 0.5 $\mu s$.}
\includegraphics[width=0.8\textwidth]{filter_1.png}
\end{cdrfigure}
%\fixme{axes of \ref{fig:soft_filter_1}  need to be labeled - description in caption is not enough.}

Beside the high-frequency software filter described above, there is also a low-frequency 
software filter which is used to select ROIs (discussed in Section~\ref{sec:decon-roi-selection}.) %the next section). 
The functional form of the low-frequency software filter is chosen to be 
\begin{equation}
F(\omega) = 1- e^{-\frac{1}{2}\cdot \left( \frac{\omega}{c} \right)^2}.
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{ROI Selection}
\label{sec:decon-roi-selection}

The region of interest (ROI) is an important technique for limiting the contribution of low-frequency 
electronic noise. The ROI selection was based on the deconvoluted results. 
Two rounds of deconvolution are performed:
\begin{itemize}
\item 2D deconvolution with the balanced Garfield-simulated field response function with a low-frequency filter (``2D deconvolution with low-frequency filter'').
\item 2D deconvolution with the balanced Garfield-simulated field response function without a low-frequency filter (``2D deconvolution'').
\end{itemize}
The first one is used to select ROIs, and the results from the second deconvolution are then 
used to obtain the final deconvoluted results. 

%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Metrics in Evaluating TPC Signal Processing}

In order to evaluate the TPC signal processing, which includes both the noise filtering and 
the charge extraction, two robust metrics can be used. % for evaluation purpose. 
They are:
\begin{itemize}
\item Equivalent Noise Charge (ENC): \\
  ENC is  basically proportional to the pedestal RMS in terms of ADC, and is a direct 
measure of the noise level in %the unit of 
electrons. It can be used to compare the 
noise levels from different experiments.
\item Deconvoluted Noise Charge after the TPC charge extraction (DNC): \\
The goal of the TPC charge extraction process is to recover the number of ionization 
electrons from the measured TPC signal. With the same procedure, the electronic noise
will also be converted. %The unit of these noise is again 
This is again measured in electrons, %which 
and so can be compared with 
the expected ionization electrons from energetic charged particles. 
The DNC depends on the ENC and on the frequency content of the noise spectrum. It also depends 
on the response function used for deconvolution, which is the primary reason 
why the induction plane DNC is much higher than the collection plane DNC. Furthermore, since
we have to rely on ROI and AB techniques to reduce the noise level for the induction plane, the
DNC also depends on the time-window length of the ROI. 
\end{itemize}
Understanding the ENC and DNC for the current-generation of experiments and for the expected 
performance of future experiments is relevant for automated event reconstruction in LArTPCs.


\begin{cdrfigure}[Residual noise vs wire length]{rms3}{The noise level in terms of the RMS value and ENC 
is plotted with respect to the wire length observed in MicroBooNE. 
This plot is taken from~\cite{noise_filter}.}
\includegraphics[width=0.75\textwidth]{RMSvsLength_after.pdf}
\end{cdrfigure}
%\fixme{incorrect figure ?!}

The ENC in MicroBooNE has been reported in~\cite{noise_filter} and plotted 
in Figure~\ref{fig:rms3}. The calculation of the DNC depends on the 
drifted-charge extraction procedure. More specifically, it depends on the field 
response, the noise level (ENC and the frequency content), and the length of the ROI. 
Figure~\ref{fig:DNC} shows the calculated DNC as a function of the time-window length 
for the second induction (V) plane, which is expected to have the smallest field 
response function  and thus the largest DNC. 

\begin{cdrfigure}[Calculation of DNC vs time window length for second induction (V) plane]{DNC}{Calculation of DNC with respect to the time window length for second induction (V) plane. 
The ENC used in this simulation is 500 electrons given the induction wire length in protoDUNE. 
The red line shows the expected signal size for a minimal ionizing particle (MIP) 
traveling 3.2 mm.}
\includegraphics[width=0.75\textwidth]{DNC.png}
\end{cdrfigure}




==> writing-standards.tex <==
%%%  \chapter{Writing Standard }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Some Instructions and Coding Standards}

A few notes:

It's helpful to add the lines of percents ahead of section delimiters for navigating through the tex document. (I have it so that it renders in color.)  Longer lines for sections, half as long for subsections, half again as long for subsubsections.

To compile the document, run pdflatex protodune-tdr

To update the Table of Contents, run that command twice.  To get everything run ./compileitdraft protodune-tdr.

The list of acronyms is copied from the CDR and will need reworking. It's controlled by some files under the common directory. We'll worry about it later!

%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{fixme}
Here's how to add a ``fixme'':
\fixme{testing}
Fixmes and line numbers will show up when you compile as draft (use ./compileitdraft protodune-tdr).

They will not show up when you compile as print (use ./compileitprint protodune-tdr).

%%%%%%%%%%%%%%
\subsubsection{Here's a subsubsection}
...with some text.

You cannot have only one section in a chapter (because that implies that the chapter doesn't need subdivision), nor can you have only one subsection in a section (for the same reason).


%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Figures}
There's an enviroment defined as cdrfigure, and all you need to do for a figure in your file is fill in the following (as it appears in the tex file, not the pdf) with the short caption, the label (without ``fig:'' at the front), the long caption and then the filename with the appropriate width:

\begin{cdrfigure}[short caption for table of figures]{label}{long caption that appears below picture}
  \includegraphics[width=0.8\textwidth]{protoDUNE_cryostat.png}
\end{cdrfigure}

The reference that points to it needs to read Figure~\ref{fig:label} (i.e., with the ``fig:'')


For tables, it's similar:

\begin{cdrtable}[short caption for table of tables]{cc}{label}{long caption to appear above table}
Header Column1 & Header Column 2 \\ \toprowrule
Row 1 & First \\ \colhline
Row 2 & Second \\ \colhline
Row 3 & Third \\
\end{cdrtable}

The third argument (reads {cc}) can use c, l, r, p{some length} but please do not include lines like `'|c|l|l|''.

The reference that points to it needs to read Table~\ref{tab:label} (i.e., with the ``tab:'')

%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{References}

In the file common/pdune-tdr-citedb.bib there are a few citations listed as examples. Please follow the format shown.  To add a reference within the text, do it like this:  ``Blah blah blah. This is described further in~\cite{cdr-annex-singleph-proto}.''

The references are not compiled with a simple run of pdflatex, you have to run the bibtex command.  It's included in the scripts compileitdraft and compileitprint.


%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{git reference}

Install git (see https://github.com/).
Clone repository (See ``Initial Clone'' in instructions at https://github.com/DUNE/document-guidance.)
General editing procedure

\begin{itemize}
\item    cd to directory into which you cloned document
\item  git pull
\item    (Edit files. Then test that document compiles.)
\item    pdflatex volume-x
\item    (Fix editing errors and retry until it compiles.)
\item    git pull (yes, again, for good measure)
\item    (If you have new files, add them.)
\item    git add volume-x/new-file.tex
\item    git add volume-x/figures/new-image-file.pdf
\item    git commit -a -m "some commit message"
\item    git push
\end{itemize}

If git pull fails:

\begin{itemize}
\item       git stash
\item      git pull
\item      git stash pop
\item      (Fix conflicts, commit and push.)
\end{itemize}

(Delete to here once you know how to do all this stuff.)

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Next Section}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{And the Next One}

%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Subsec 1}


%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Subsec 2}



